R-vine Models for Spatial Time Series with an Application to Daily Mean Temperature

We introduce an extension of R-vine copula models for the purpose of spatial dependency modeling and model based prediction at unobserved locations. The newly derived spatial R-vine model combines the flexibility of vine copulas with the classical geostatistical idea of modeling spatial dependencies by means of the distances between the variable locations. In particular the model is able to capture non-Gaussian spatial dependencies. For the purpose of model development and as an illustration we consider daily mean temperature data observed at 54 monitoring stations in Germany. We identify a relationship between the vine copula parameters and the station distances and exploit it in order to reduce the huge number of parameters needed to parametrize a 54-dimensional R-vine model needed to fit the data. The new distance based model parametrization results in a distinct reduction in the number of parameters and makes parameter estimation and prediction at unobserved locations feasible. The prediction capabilities are validated using adequate scoring techniques, showing a better performance of the spatial R-vine copula model compared to a Gaussian spatial model.

==> Sections/Composite.tex <==

\section[Spatial composite vine models]{Spatial composite vine models}\label{sec:composite}

The previous section was a straigthforward approach to model spatial dependencies based on vine copula models by embedding spatial information into the parametrization of an R-vine model. This chapter is going to follow a different approach which composes several local dependency models by means of a composite likelihood, where the modeling of these local dependencies is carried out by C-vines. For the purpose of composite likelihood methods we refer to \citet*[][]{varin11}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Section 01 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Composite likelihood methods}\label{sec:comp:like}
%
%In order to have the necessary background to be able to understand the models presented in the following, we briefly provide some theoretical aspects on \emph{composite likelihood methods}. For this purpose we refer to \citet*[][]{varin11}, who give a broad overview on these methods.
%
%Composite likelihood methods are inferential statistics methods. The main idea of these methods is the composition of a composite likelihood function as a product of potentially dependent likelihoods corresponding to certain parts of the model under consideration. Due to the fact that the single likelihoods are not necessarily independent, the composite likelihood can be considered as the likelihood of a misspecified model. The usage of such misspecified models is most often motivated computationally.
%
%Let us now formally define the composite likelihood. To this end, let $\bY$ be an $m$-dimensional random vector with multivariate probability density function $f(\by\sepi\btheta)$, where $\btheta$ is a $p$-dimensional parameter vector. Moreover we consider $K$ events $\xn{\calA}{K}$ and weights $w_k>0$, $\iN{k}{K}$, related to these events. Furthermore, let the likelihoods corresponding to the events $\calA_k$, $\iN{k}{K}$, be denoted by $\Lik{k}{\btheta}{\by} \propto f(\by\in\calA_k\sepi\btheta)$, $\iN{k}{K}$. Then the \emph{composite likelihood} is defined as
%\beqo
%	\Lik{C}{\btheta}{\by}	=	\prod_{k=1}^{K}\left[\Lik{k}{\btheta}{\by}\right]^{w_k}.
%\eeqo
%Following the composite log-likelihood is given and denoted by
%\beqo
%	\cll{}{\btheta}{\by}	\coloneqq \ln \Lik{C}{\btheta}{\by}	=	\sum_{k=1}^{K}{w_k}\ln \left[\Lik{k}{\btheta}{\by}\right]	=	\sum_{k=1}^{K}{w_k}\ll{k}{\btheta}{\by}.
%\eeqo
%
%The idea behind the weights $w_k$, $\iN{k}{K}$, is to improve the efficiency of maximum composite likelihood estimation. Their selection depends on the specific problem.
%
%\citet[][]{varin11} distinguish between composite conditional and composite marginal likelihoods. Whereas a composite conditional  likelihood is composed out of conditional densities, a composite marginal likelihood is based on marginal densities. Since we are going to use a composite marginal likelihood, we focus on this variant in the following.
%
%A straightforward composite marginal likelihood is the product of the univariate marginal densities $f(y_r\sepi\btheta)$, $\iN{r}{m}$. Due to this structure, this kind of likelihood does not allow to access parameters which are related to the dependence of the components of $\bY$. In order to do so, multivariate marginal densities have to be taken into consideration. A popular example is the so called pairwise likelihood
%\beqo
%	\Lik{\text{pair}}{\btheta}{\by}	=	\prod_{r=1}^{m-1}\prod_{s=r+1}^{m}f(y_r,y_s\sepi\btheta),
%\eeqo
%but it is also possible to use products of higher dimensional marginal densities, what we are going to do in the following.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Section 02 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Composite vine model}\label{sec:CVM}

Now we are going to propose our own composite likelihood model in the area of spatial dependence modeling. For this purpose let us again consider the copula data $\bu^1,\ldots,\bu^d$ with $\bu^s=(u^s_{1},\ldots,u^s_{N})\T$, $\iN{s}{d}$. To model the dependence of this data, we are going to set up a composite likelihood model which is composed out of the densities corresponding to $d$ $4$-dimensional C-vines numbered $1,\ldots,d$, i.e. we consider one C-vine for every variable $\bu^s$, $\iN{s}{d}$. The first root node of every C-vine $\iN{s}{d}$ complies with the number $s$ of the C-vine. In other words, the C-vines are numbered according to their first root nodes. For each C-vine $s$ we select the variable $p_s$ with the shortest distance to the first root node $s$ as the second root, the variable $q_s$ with the second shortest distance as the third root and the variable $r_s$ with the third shortest distance as the forth variable of the C-vine. Now we have uniquely fixed the tree structure of all $d$ C-vines in the model. Figure \ref{fig:cvines} gives a graphical representation of these C-vines.

\begin{figure}[htb]
	\centerline{
		\entrymodifiers={++[o][F]}
		%\SelectTips{cm}{}
		\xymatrix @+2pc {
		*{\tree_1}						& *\txt{}									&	*{\tree_2}	& *\txt{}											&	*{\tree_3}							\\
		p_s	\ar@{-}[d]_{sp_s}	& q_s \ar@{-}[dl]_{sq_s}	&	sp_s				& sq_s \ar@{-}[l]_{p_sq_s|s}	& p_sq_s|s \ar@{-}[d]^{q_sr_s|sp_s}	\\
		s											& r_s \ar@{-}[l]_{sr_s}		&	*\txt{}			& sr_s \ar@{-}[ul]^{p_sr_s|s}	& p_sr_s|s										\\
		}
	}
	\caption{Structure of all C-vines $\iN{s}{d}$ composing the composite likelihood model.}
	\label{fig:cvines}
\end{figure}

Moreover, the families of the bivariate copulae corresponding to the edges of the $d$ C-vines have to be specified. They are determined by means of a sequential selection algorithm, for each single C-vine.

Finally, as all necessary components of the C-vines $\iN{s}{d}$ are established, we are able to state their likelihoods. They are given as
\begin{align*}
	\Lik{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}	& =	\cop{s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t} \sepi \btheta_s, \bnu_s}	\\*
	& = \cop{sp_s}{u^{s}_{t},u^{p_s}_{t} \sepi \te_{sp_s},\nu_{sp_s}} \cdot \cop{sq_s}{u^{s}_{t},u^{q_s}_{t} \sepi \te_{sq_s},\nu_{sq_s}}	\\*
	& \cdot	\cop{sr_s}{u^{s}_{t},u^{r_s}_{t} \sepi \te_{sr_s},\nu_{sr_s}}	\\*
	& \cdot	\cop{p_sq_s;s}{\breve{u}^{p_s}_{t},\breve{u}^{q_s}_{t} \sepi \te_{p_sq_s|s},\nu_{p_sq_s|s}} \cdot \cop{p_sr_s;s}{\breve{u}^{p_s}_{t},\breve{u}^{r_s}_{t} \sepi \te_{p_sr_s|s},\nu_{p_sr_s|s}}	\\*
	& \cdot	\cop{q_sr_s;sp_s}{\check{u}^{q_s}_{t},\check{u}^{r_s}_{t} \sepi \te_{q_sr_s|sp_s},\nu_{q_sr_s|sp_s}}
\end{align*}
where
\beqo
	\breve{u}^{o}_{t} =	F(u^{o}_{t} \sep u^{s}_{t}) =	\partialderiv{u^{s}_{t}} \Cop{os}{u^{o}_{t},u^{s}_{t} \sepi \te_{so},\nu_{so}}, \quad o=p_s,q_s,r_s,
\eeqo
\beqo
	\check{u}^{o}_{t} =	F(u^{o}_{t} \sep u^{s}_{t},u^{p_s}_{t}) = \partialderiv{\breve{u}^{p_s}_{t}} \Cop{op_s;s}{\breve{u}^{o}_{t},\breve{u}^{p_s}_{t} \sepi \te_{p_so|s},\nu_{p_so|s}}, \quad o=q_s,r_s,
\eeqo
and
\begin{align*}
	\btheta_s	& =	\left(\te_{sp_s}, \te_{sq_s}, \te_{sr_s}, \te_{p_sq_s|s}, \te_{p_sr_s|s}, \te_{q_sr_s|sp_s}\right)\T,	\\
	\bnu_s	& =	\left(\nu_{sp_s}, \nu_{sq_s}, \nu_{sr_s}, \nu_{p_sq_s|s}, \nu_{p_sr_s|s}, \nu_{q_sr_s|sp_s}\right)\T.	\\
\end{align*}
Note that the second parameter $\nu_{ij|\ldots}$ of the bivariate copula is only needed in the case of a Student-$t$ copula, for the respective degrees of freedom. Otherwise the bivariate copula does not depend on $\nu_{ij|\ldots}$ and we omit this parameter or set it simply to zero. Note furthermore, that in trees of order one it holds for the parameters, that $\te_{ij}=\te_{ji}$ and $\nu_{ij}=\nu_{ji}$, $\iN{i}{d}$, $\iN{j}{d}$, since each edge $\left\{i,j\right\}$ may occur in up to two of the $d$ C-vines composing the model.

In order to be able to set up the composite likelihood, it remains to specify the weights $w_s$, $\iN{s}{d}$. We define them as the reciprocal value of the number counts
\beqo
	n_s \coloneqq \#\left\{k: s \mbox{ is included in C-vine }k\right\},\ \iN{s}{d},
\eeqo
of C-vines which include $\iN{s}{d}$, i.e. we define
\beqo
	w_s \coloneqq \frac{1}{n_s}.
\eeqo

All in all, this results in the composite likelihood
\beqo
	\Lik{\text{CVM}}{\btheta^\text{CVM}, \bnu^\text{CVM}}{\bu^1,\ldots,\bu^d}	=	\prodsd\prodtN\left[\Lik{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}\right]^{w_s}
\eeqo
and accordingly in the composite log-likelihood
\beqq\label{eq:compll}
	\cll{\text{CVM}}{\btheta^\text{CVM}, \bnu^\text{CVM}}{\bu^1,\ldots,\bu^d}	=	\sumsd\sumtN{w_s}\ll{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}},
\eeqq
where
\beqo
	\ll{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}	=	\ln \Lik{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}
\eeqo
and where
\begin{align*}
	\btheta^\text{CVM}	& =	\left\{\theta: \theta\in\btheta_s, \iN{s}{d}\right\},	\\
	\bnu^\text{CVM}	& =	\left\{\nu: \nu\in\bnu_s, \iN{s}{d}\right\}.
\end{align*}
We call the above model a (three neighbors) \emph{composite vine model (CVM)}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Section 03 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A composite vine model for mean temperature}\label{sec:CVM:app}

Eventually we are going to investigate the mean temperature data set with the help of the above model. In a first step we have to select the structure of the composite vine model. This involves amongst others the selection of the $54$ C-vines. They are selected as described in Section \ref{sec:CVM}. The result of this selection is given in Table \ref{tab:CVM:roots}. Moreover we have to determine adequate families for the $6\cdot54=324$ bivariate copulae corresponding to the edges of the previously chosen C-vines. To this end we allow for Gaussian ($\Phi$), Student-$t$ (t), Clayton (C), Gumbel (G) and Frank (F) copulae, without specifying in detail if a rotated version of the respective copula is used or not. The exact rotation type will be fixed later on, when the respective parameters are estimated. We achieve families as given in Table \ref{tab:CVM:fam}. This results in a parametrization with $464$ parameters.

%% latex table generated in R 2.15.0 by xtable 1.7-1 package
%% Sat Jun 08 18:35:38 2013
%\begin{table}[htb]
%\centering
%\begin{tabular}{rrrr||rrrr||rrrr}
	%$s$ & $p_s$ & $q_s$ & $r_s$ & $s$ & $p_s$ & $q_s$ & $r_s$ & $s$ & $p_s$ & $q_s$ & $r_s$ \\ 
  %\hline
	%\hline
	%1 & 4 & 49 & 40 & 19 & 26 & 6 & 35 & 37 & 39 & 27 & 43 \\ 
  %2 & 24 & 10 & 29 & 20 & 33 & 24 & 23 & 38 & 30 & 31 & 12 \\ 
  %3 & 17 & 31 & 36 & 21 & 32 & 50 & 9 & 39 & 37 & 43 & 41 \\ 
  %4 & 1 & 40 & 23 & 22 & 6 & 50 & 7 & 40 & 4 & 52 & 1 \\ 
  %5 & 36 & 12 & 3 & 23 & 8 & 20 & 10 & 41 & 53 & 54 & 29 \\ 
  %6 & 22 & 16 & 50 & 24 & 20 & 29 & 2 & 42 & 15 & 37 & 43 \\ 
  %7 & 22 & 9 & 21 & 25 & 45 & 34 & 48 & 43 & 53 & 39 & 41 \\ 
  %8 & 23 & 18 & 10 & 26 & 19 & 31 & 3 & 44 & 52 & 32 & 49 \\ 
  %9 & 21 & 46 & 7 & 27 & 51 & 37 & 39 & 45 & 25 & 48 & 34 \\ 
  %10 & 18 & 8 & 2 & 28 & 51 & 27 & 14 & 46 & 9 & 21 & 32 \\ 
  %11 & 30 & 7 & 9 & 29 & 35 & 24 & 41 & 47 & 51 & 34 & 54 \\ 
  %12 & 5 & 38 & 31 & 30 & 38 & 11 & 7 & 48 & 45 & 25 & 36 \\ 
  %13 & 34 & 17 & 36 & 31 & 3 & 38 & 26 & 49 & 1 & 52 & 40 \\ 
  %14 & 28 & 47 & 45 & 32 & 21 & 50 & 44 & 50 & 6 & 16 & 22 \\ 
  %15 & 42 & 43 & 37 & 33 & 16 & 20 & 6 & 51 & 47 & 27 & 28 \\ 
  %16 & 33 & 6 & 50 & 34 & 13 & 25 & 47 & 52 & 40 & 44 & 49 \\ 
  %17 & 3 & 13 & 36 & 35 & 29 & 54 & 24 & 53 & 43 & 41 & 29 \\ 
  %18 & 10 & 8 & 23 & 36 & 5 & 17 & 13 & 54 & 41 & 35 & 13 \\ 
%\end{tabular}
%\caption[Variables composing the $54$ C-vines of the (spatial) composite vine model (mean temperature data).]{Variables composing the $54$ C-vines of the (spatial) composite vine model on the $54$ observation stations of our mean temperature data set.} 
%\label{tab:CVM:roots}
%\end{table}

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Thu Aug 15 00:23:26 2013
\begin{table}[htb]
\centering
\begin{tabular}{rrrr||rrrr||rrrr||rrrr}
	$s$ & $p_s$ & $q_s$ & $r_s$ & $s$ & $p_s$ & $q_s$ & $r_s$ & $s$ & $p_s$ & $q_s$ & $r_s$ & $s$ & $p_s$ & $q_s$ & $r_s$ \\ 
  \hline
	\hline
	1 & 4 & 49 & 40 & 15 & 42 & 43 & 37 & 29 & 35 & 24 & 41 & 43 & 53 & 39 & 41 \\ 
  2 & 24 & 10 & 29 & 16 & 33 & 6 & 50 & 30 & 38 & 11 & 7 & 44 & 52 & 32 & 49 \\ 
  3 & 17 & 31 & 36 & 17 & 3 & 13 & 36 & 31 & 3 & 38 & 26 & 45 & 25 & 48 & 34 \\ 
  4 & 1 & 40 & 23 & 18 & 10 & 8 & 23 & 32 & 21 & 50 & 44 & 46 & 9 & 21 & 32 \\ 
  5 & 36 & 12 & 3 & 19 & 26 & 6 & 35 & 33 & 16 & 20 & 6 & 47 & 51 & 34 & 54 \\ 
  6 & 22 & 16 & 50 & 20 & 33 & 24 & 23 & 34 & 13 & 25 & 47 & 48 & 45 & 25 & 36 \\ 
  7 & 22 & 9 & 21 & 21 & 32 & 50 & 9 & 35 & 29 & 54 & 24 & 49 & 1 & 52 & 40 \\ 
  8 & 23 & 18 & 10 & 22 & 6 & 50 & 7 & 36 & 5 & 17 & 13 & 50 & 6 & 16 & 22 \\ 
  9 & 21 & 46 & 7 & 23 & 8 & 20 & 10 & 37 & 39 & 27 & 43 & 51 & 47 & 27 & 28 \\ 
  10 & 18 & 8 & 2 & 24 & 20 & 29 & 2 & 38 & 30 & 31 & 12 & 52 & 40 & 44 & 49 \\ 
  11 & 30 & 7 & 9 & 25 & 45 & 34 & 48 & 39 & 37 & 43 & 41 & 53 & 43 & 41 & 29 \\ 
  12 & 5 & 38 & 31 & 26 & 19 & 31 & 3 & 40 & 4 & 52 & 1 & 54 & 41 & 35 & 13 \\ 
  13 & 34 & 17 & 36 & 27 & 51 & 37 & 39 & 41 & 53 & 54 & 29 &  &  &  &  \\ 
	14 & 28 & 47 & 45 & 28 & 51 & 27 & 14 & 42 & 15 & 37 & 43 &  &  &  &  \\ 
\end{tabular}
\caption[Variables composing the $54$ C-vines of the (spatial) composite vine model (mean temperature data).]{Variables composing the $54$ C-vines of the (spatial) composite vine model on the $54$ observation stations of our mean temperature data set.} 
\label{tab:CVM:roots}
\end{table}

%% latex table generated in R 2.15.0 by xtable 1.7-1 package
%% Sat Jun 29 23:12:43 2013
%\begin{table}[htbp]
%\centering
%\begin{tabular}{r|rrrrrr||r|rrrrrr}
	%$s$ & \rotatebox{90}{$sp_s$} & \rotatebox{90}{$sq_s$} & \rotatebox{90}{$sr_s$} & \rotatebox{90}{$p_sq_s|s$} & \rotatebox{90}{$p_sr_s|s$} & \rotatebox{90}{$q_sr_s|sp_s$} & $s$ & \rotatebox{90}{$sp_s$} & \rotatebox{90}{$sq_s$} & \rotatebox{90}{$sr_s$} & \rotatebox{90}{$p_sq_s|s$} & \rotatebox{90}{$p_sr_s|s$} & \rotatebox{90}{$q_sr_s|sp_s$} \\ 
  %\hline
	%\hline
	%1 & t & t & t & t & t & t & 28 & t & t & t & t & t & G \\ 
  %2 & t & t & t & t & t & t & 29 & t & t & t & F & t & t \\ 
  %3 & t & t & t & t & t & C & 30 & t & t & t & t & t & t \\ 
  %4 & t & t & t & t & t & G & 31 & t & t & t & t & t & t \\ 
  %5 & t & t & t & t & t & t & 32 & t & t & G & t & t & G \\ 
  %6 & t & t & t & F & t & t & 33 & t & t & t & t & t & C \\ 
  %7 & t & t & t & C & F & t & 34 & t & t & t & F & t & t \\ 
  %8 & t & t & t & G & t & t & 35 & t & t & t & t & t & t \\ 
  %9 & t & t & t & t & t & t & 36 & t & t & t & G & t & t \\ 
  %10 & t & t & t & t & t & t & 37 & t & t & t & t & t & t \\ 
  %11 & t & t & t & t & F & t & 38 & t & t & t & t & t & t \\ 
  %12 & t & t & t & t & t & t & 39 & t & t & t & t & t & t \\ 
  %13 & t & t & t & t & G & t & 40 & t & t & t & C & t & t \\ 
  %14 & t & t & t & t & t & t & 41 & t & t & t & t & t & G \\ 
  %15 & t & t & G & $\Phi$ & t & $\Phi$ & 42 & t & t & t & t & t & $\Phi$ \\ 
  %16 & t & t & t & t & t & t & 43 & t & t & t & G & t & t \\ 
  %17 & t & t & t & t & t & t & 44 & t & G & t & t & t & t \\ 
  %18 & t & t & t & t & t & t & 45 & t & t & t & F & t & t \\ 
  %19 & t & t & t & t & t & C & 46 & t & t & G & t & G & t \\ 
  %20 & t & t & t & t & t & G & 47 & t & t & t & C & t & t \\ 
  %21 & t & t & t & t & t & C & 48 & t & t & t & t & t & t \\ 
  %22 & t & t & t & t & t & t & 49 & t & t & t & t & t & t \\ 
  %23 & t & t & t & t & t & t & 50 & t & t & t & t & t & t \\ 
  %24 & t & t & t & t & t & t & 51 & t & t & t & t & t & t \\ 
  %25 & t & t & t & t & t & t & 52 & t & t & t & t & t & t \\ 
  %26 & t & t & t & t & t & t & 53 & t & t & t & t & t & t \\ 
  %27 & t & t & t & t & t & t & 54 & t & t & t & t & t & t \\ 
%\end{tabular}
%\caption[Families of the copulae of the C-vines $\iN{s}{54}$ of the (spatial) composite vine model for our mean temperature data set.]{Families of the copulae of the C-vines $\iN{s}{54}$ of the (spatial) composite vine model for our mean temperature data set.} 
%\label{tab:CVM:fam}
%\end{table}

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Thu Aug 15 00:29:50 2013
\begin{table}[htb]
\centering
\small\begin{tabular}{r|rrrrrr||r|rrrrrr||r|rrrrrr}
	$s$ & \rotatebox{90}{$sp_s$} & \rotatebox{90}{$sq_s$} & \rotatebox{90}{$sr_s$} & \rotatebox{90}{$p_sq_s|s$} & \rotatebox{90}{$p_sr_s|s$} & \rotatebox{90}{$q_sr_s|sp_s$} & $s$ & \rotatebox{90}{$sp_s$} & \rotatebox{90}{$sq_s$} & \rotatebox{90}{$sr_s$} & \rotatebox{90}{$p_sq_s|s$} & \rotatebox{90}{$p_sr_s|s$} & \rotatebox{90}{$q_sr_s|sp_s$} & $s$ & \rotatebox{90}{$sp_s$} & \rotatebox{90}{$sq_s$} & \rotatebox{90}{$sr_s$} & \rotatebox{90}{$p_sq_s|s$} & \rotatebox{90}{$p_sr_s|s$} & \rotatebox{90}{$q_sr_s|sp_s$} \\ 
  \hline
	\hline
	1 & t & t & t & t & t & t & 19 & t & t & t & t & t & C & 37 & t & t & t & t & t & t \\ 
  2 & t & t & t & t & t & t & 20 & t & t & t & t & t & G & 38 & t & t & t & t & t & t \\ 
  3 & t & t & t & t & t & C & 21 & t & t & t & t & t & C & 39 & t & t & t & t & t & t \\ 
  4 & t & t & t & t & t & G & 22 & t & t & t & t & t & t & 40 & t & t & t & C & t & t \\ 
  5 & t & t & t & t & t & t & 23 & t & t & t & t & t & t & 41 & t & t & t & t & t & G \\ 
  6 & t & t & t & F & t & t & 24 & t & t & t & t & t & t & 42 & t & t & t & t & t & $\Phi$ \\ 
  7 & t & t & t & C & F & t & 25 & t & t & t & t & t & t & 43 & t & t & t & G & t & t \\ 
  8 & t & t & t & G & t & t & 26 & t & t & t & t & t & t & 44 & t & G & t & t & t & t \\ 
  9 & t & t & t & t & t & t & 27 & t & t & t & t & t & t & 45 & t & t & t & F & t & t \\ 
  10 & t & t & t & t & t & t & 28 & t & t & t & t & t & G & 46 & t & t & G & t & G & t \\ 
  11 & t & t & t & t & F & t & 29 & t & t & t & F & t & t & 47 & t & t & t & C & t & t \\ 
  12 & t & t & t & t & t & t & 30 & t & t & t & t & t & t & 48 & t & t & t & t & t & t \\ 
  13 & t & t & t & t & G & t & 31 & t & t & t & t & t & t & 49 & t & t & t & t & t & t \\ 
  14 & t & t & t & t & t & t & 32 & t & t & G & t & t & G & 50 & t & t & t & t & t & t \\ 
  15 & t & t & G & $\Phi$ & t & $\Phi$ & 33 & t & t & t & t & t & C & 51 & t & t & t & t & t & t \\ 
  16 & t & t & t & t & t & t & 34 & t & t & t & F & t & t & 52 & t & t & t & t & t & t \\ 
  17 & t & t & t & t & t & t & 35 & t & t & t & t & t & t & 53 & t & t & t & t & t & t \\ 
  18 & t & t & t & t & t & t & 36 & t & t & t & G & t & t & 54 & t & t & t & t & t & t \\ 
\end{tabular}
\caption[Families of the copulae of the C-vines $\iN{s}{54}$ of the (spatial) composite vine model for our mean temperature data set.]{Families of the copulae of the C-vines $\iN{s}{54}$ of the (spatial) composite vine model for our mean temperature data set.} 
\label{tab:CVM:fam}
\end{table}

Figure \ref{fig:GermanySCVM} illustrates the achieved model structure. On the one hand the numbered circles indicate the locations of the $54$ observation stations $\iN{s}{54}$ summarized in Table \ref{tab:stations}. Their circumference and color represents the numbers $n_s$, $\iN{s}{54}$, of C-vines in which the respective nodes are included, i.e. the inverse of the respective weights $w_s$, $\iN{s}{54}$, according to the scale defined at the left bottom of the figure. On the other hand the lines indicate all C-vine edges that occur in the first trees of the C-vines $\iN{s}{54}$. Dotted lines represent edges that occur only once, whereas dashed lines represent edges that occur in the first tree of two C-vines.

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{Figures/GermanySCVM.pdf}
	\caption[Visualization of the model structure of a (spatial) composite vine model (mean temperature data).]{Visualization of the model structure of a (spatial) composite vine model on the $54$ observation stations of our mean temperature data set.}
	\label{fig:GermanySCVM}
\end{figure}

For the mean temperature data set numerical maximization of the composite log-likelihood \eqref{eq:compll}, whose structure and components where specified above, yields a maximum composite log-likelihood of $\cll{\text{CVM}}{\wh\btheta^\text{CVM}, \wh\bnu^\text{CVM}}{\bu^1,\ldots,\bu^d} = 42106.41$. The respective AIC and BIC are given by $\AIC_\text{CVM} = -83222.8$ and $\BIC_\text{CVM} = -80749.5$.

\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Section 04 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Spatial composite vine models}\label{sec:SCVM}

Now we are going to enhance our composite vine model in terms of parameter number reduction by utilization of additionally available spatial information on the considered variables. %, in order to further reduce the number of parameters in the model.
Therefore we follow a similar reparametrization approach as in the section about spatial R-vine models (Section \ref{sec:svines}).

This time we have to consider reparametrizations of the parameters $\btheta^\text{CVM}$ of the composite vine model. Since these reparametrizations differ from the ones in Section \ref{sec:svines}, we are going to state them in detail in the following. Furthermore a reparametrization of the parameters $\bnu^\text{CVM}$ is needed.% We will call the reparametrized (three neighbors) composite vine model a (three neighbors) \emph{spatial composite vine model}.

Once again we will initiate our model building process by a tree-wise exploratory analysis of the dependence of the parameters $\btheta^\text{CVM}$ on the distances and elevation differences occurring in the C-vines composing the composite vine model on the mean temperature data. To this end we again calculate and transform the Kendall's $\tau$'s corresponding to the variable pairs specified by the $54$ C-vines and plot their transformations against the respective logarithmized distances and logarithmized elevation differences.

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{Figures/SpatialCompTDE01.pdf}
	\caption[Scatter plots: $\text{F}_z(\wh\tau_{s,o})$ against $\ln\left(d_{s,o}\right)$ and $\ln\left(e_{s,o}\right)$ (Tree 1).]{Scatter plots of $\text{F}_z(\wh\tau_{s,o})$ against $\ln\left(d_{s,o}\right)$ and $\ln\left(e_{s,o}\right)$, respectively, where $o=p_s,q_s,r_s$ and $\iN{s}{54}$ (Tree 1).}
	\label{fig:SCVM:tree1}
\end{figure}

The respective plots for the first trees of the C-vines are depicted in Figure \ref{fig:SCVM:tree1}. $54$ trees $\iN{s}{54}$, each consisting of the three edges $\{s,p_s\}$, $\{s,q_s\}$ and $\{s,r_s\}$, yield $162$ points per plot, where a big share of the previously mentioned edges occur twice, i.e. lots of the points of the plot are twofold. These twofold points are highlighted in gray. Both plots, the plot of the Fisher z-transformed Kendall's $\tau$'s against the logarithmized distances and the plot against the logarithmized elevation differences, suggest the inclusion of the predictors $d_{s,o}$ and $e_{s,o}$ into the model for the parameters of the first tree, where $o=p_s,q_s,r_s$.

For the second and third trees we additionally have to consider the distances and elevation differences to the conditioning variables of the respective copulae. This time there is an ordering of the conditioning variables, since there is an ordering of the root nodes of the C-vines, i.e. the variables $s$ enter the conditioning set before the variables $p_s$, $\iN{s}{54}$. Hence we do not have to define means according to our investigations in Subsection \ref{sec:prem:ana}, i.e. the distances and elevation differences corresponding to the edges of the third trees can be considered separately.

Figure \ref{fig:SCVM:tree2} shows the six scatter plots of the Fisher z-transformed Kendall's $\tau$'s $\wh\tau_{p_s,o|s}$ against the logarithmized distances and elevation differences of the station pairs $\{p_s,o\}$, $\{p_s,s\}$ and $\{o,s\}$, where $o=q_s,r_s$. We observe evident linear trends for the distances. The three plots for the elevation differences exhibit only slight slopes of the regression lines and seemingly random broad scatter around this line.

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{Figures/SpatialCompTDE02.pdf}
	\caption[Scatter plots:  $\text{F}_z(\wh\tau_{p_s,o|s})$ against $\ln\left(d_{p_s,o}\right)$, $\ln\left(e_{p_s,o}\right)$, $\ln\left(d_{p_s,s}\right)$, $\ln\left(e_{p_s,s}\right)$, $\ln\left(d_{o,s}\right)$ and $\ln\left(e_{o,s}\right)$ (Tree 2).]{Scatter plots of  $\text{F}_z(\wh\tau_{p_s,o|s})$ against $\ln\left(d_{p_s,o}\right)$, $\ln\left(e_{p_s,o}\right)$, $\ln\left(d_{p_s,s}\right)$, $\ln\left(e_{p_s,s}\right)$, $\ln\left(d_{o,s}\right)$ and $\ln\left(e_{o,s}\right)$, respectively, where $o=q_s,r_s$ and $\iN{s}{54}$ (Tree 2).}
	\label{fig:SCVM:tree2}
\end{figure}

The plots for the third C-vine trees are given in Figure \ref{fig:SCVM:tree3}. In accordance with the lower trees, the Fisher z-transformed Kendall's $\tau$'s show an evident linear dependence with respect to the logarithmized distances corresponding to the  conditioned variables, whereas the regression line slopes of most of the remaining plots are rather negligible.

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{Figures/SpatialCompTDE03.pdf}
	\caption[Scatter plots: $\text{F}_z(\wh\tau_{q_s,r_s|sp_s})$ against $\ln\left(d_{q_s,r_s}\right)$, $\ln\left(e_{q_s,r_s}\right)$, $\ln\left(d_{q_s,s}\right)$, $\ln\left(e_{q_s,s}\right)$, $\ln\left(d_{q_s,p_s}\right)$, $\ln\left(e_{q_s,p_s}\right)$, $\ln\left(d_{r_s,s}\right)$, $\ln\left(e_{r_s,s}\right)$, $\ln\left(d_{r_s,p_s}\right)$ and $\ln\left(e_{r_s,p_s}\right)$ (Tree 3).]{Scatter plots of $\text{F}_z(\wh\tau_{q_s,r_s|sp_s})$ against $\ln\left(d_{q_s,r_s}\right)$, $\ln\left(e_{q_s,r_s}\right)$, $\ln\left(d_{q_s,s}\right)$, $\ln\left(e_{q_s,s}\right)$, $\ln\left(d_{q_s,p_s}\right)$, $\ln\left(e_{q_s,p_s}\right)$, $\ln\left(d_{r_s,s}\right)$, $\ln\left(e_{r_s,s}\right)$, $\ln\left(d_{r_s,p_s}\right)$ and $\ln\left(e_{r_s,p_s}\right)$, respectively, where $\iN{s}{54}$ (Tree 3).}
	\label{fig:SCVM:tree3}
\end{figure}

The above investigations of the mean temperature data set give us an idea, which distances and elevation differences might play an important role in the reparametrization of our composite vine model. In order to be able to select an adequate reparametrization we set up different reparametrizations of the form
\begin{align}\label{eq:SCVM:repar}
	\wt\te_{io_1}	&	= \itau\left(\Fzi \left(h_{1}^{\text{mod}}(i,o_1|\bbeta_{\text{mod},1})\right);t_{io_1}\right),	\nonumber\\*
	\wt\te_{jo_2|i}	&	= \itau\left(\Fzi \left(h_{2}^{\text{mod}}(i,j,o_2|\bbeta_{\text{mod},2})\right);t_{jo_2|i}\right),	\\*
	\wt\te_{ko_3|ij}	&	= \itau\left(\Fzi \left(h_{3}^{\text{mod}}(i,j,k,o_3|\bbeta_{\text{mod},3})\right);t_{ko_3|ij}\right),	\nonumber
\end{align}
where 'mod' stands for the reparametrization under consideration. Selection of
	$i	=	s$,	$j	=	p_s$,	$k	=	q_s$,	$o_1	=	p_s,q_s,r_s$,	$o_2	=	q_s,r_s$	and	$o_3	=	r_s$, for all $\iN{s}{54}$, yields formulas for all parameters composing $\btheta$. The \emph{model functions} $h_{l}^{\text{mod}}$, $l=1,2,3$, for different reparametrizations 'mod' will be specified in detail, below. Due to the structural similarity of these reparametrizations to the reparametrizations defined in Section \ref{sec:svines}, we adopt the names applied there.

First of all we consider the \emph{full reparametrization} (full), where the model functions $h_{l}^{\text{mod}}$, $l=1,2,3$, in \eqref{eq:SCVM:repar} are given as
\begin{align*}
	h_{1}^{\text{full}}\left(i,o_1|\bbeta_{\text{full},1}\right) = \beta_{1,0}^{\text{full}}	&	+ \beta_{1,1}^{\text{full}}\lnf{d_{i,o_1}} + \beta_{1,2}^{\text{full}}\lnf{e_{i,o_1}},	\\
	h_{2}^{\text{full}}\left(i,j,o_2|\bbeta_{\text{full},2}\right) = \beta_{2,0}^{\text{full}}	&	+ \beta_{2,1}^{\text{full}}\lnf{d_{j,o_2}} + \beta_{2,2}^{\text{full}}\lnf{d_{j,i}}	+ \beta_{2,3}^{\text{full}}\lnf{d_{o_2,i}}	\\*
		&	+ \beta_{2,4}^{\text{full}}\lnf{e_{j,o_2}} + \beta_{2,5}^{\text{full}}\lnf{e_{j,i}}	 + \beta_{2,6}^{\text{full}}\lnf{e_{o_2,i}},	\\
	h_{3}^{\text{full}}\left(i,j,k,o_3|\bbeta_{\text{full},3}\right) = \beta_{3,0}^{\text{full}}	&	+ \beta_{3,1}^{\text{full}}\lnf{d_{k,o_3}}	+ \beta_{3,2}^{\text{full}}\lnf{d_{k,i}}	+ \beta_{3,3}^{\text{full}}\lnf{d_{k,j}}	\\*
		&	+ \beta_{3,4}^{\text{full}}\lnf{d_{o_3,i}}	+ \beta_{3,5}^{\text{full}}\lnf{d_{o_3,j}}	\\*
		&	+ \beta_{3,6}^{\text{full}}\lnf{e_{k,o_3}}	+ \beta_{3,7}^{\text{full}}\lnf{e_{k,i}}	+ \beta_{3,8}^{\text{full}}\lnf{e_{k,j}}	\\*
		&	+ \beta_{3,9}^{\text{full}}\lnf{e_{o_3,i}} + \beta_{3,10}^{\text{full}}\lnf{e_{o_3,j}},
\end{align*}
and it holds
\begin{align*}
	\bbeta_{\text{full},1}	&	= \left(\beta_{1,0}^{\text{full}}, \beta_{1,1}^{\text{full}}, \beta_{1,2}^{\text{full}}\right)\T \in \R^{3},	\\*
	\bbeta_{\text{full},2}	&	= \left(\beta_{2,0}^{\text{full}}, \ldots, \beta_{2,6}^{\text{full}}\right)\T \in \R^{7},	\\*
	\bbeta_{\text{full},3}	&	= \left(\beta_{3,0}^{\text{full}}, \ldots, \beta_{3,10}^{\text{full}}\right)\T \in \R^{11},
\end{align*}
for the corresponding parameter vectors. The full reparametrization involves all available predictors. Its parameters are summarized in the vector
\beqo
	\bbeta_{\text{full}}^{\text{SCVM}} = \left(\bbeta_{\text{full},1}\T,\bbeta_{\text{full},2}\T,\bbeta_{\text{full},3}\T\right)\T \in \R^{n_\text{par}^\text{full}},
\eeqo
where $n_\text{par}^\text{full} = 3+7+11 = 21$.

Next we give the model functions $h_{l}^{\text{mod}}$, $l=1,2,3$, for the \emph{distance reparametrization} (dist). They are defined as
\begin{align*}
	h_{1}^{\text{dist}}\left(i,o_1|\bbeta_{\text{dist},1}\right) = \beta_{1,0}^{\text{dist}}	&	+ \beta_{1,1}^{\text{dist}}\lnf{d_{i,o_1}},	\\
	h_{2}^{\text{dist}}\left(i,j,o_2|\bbeta_{\text{dist},2}\right) = \beta_{2,0}^{\text{dist}}	&	+ \beta_{2,1}^{\text{dist}}\lnf{d_{j,o_2}}	+ \beta_{2,2}^{\text{dist}}\lnf{d_{j,i}}	+ \beta_{2,3}^{\text{dist}}\lnf{d_{o_2,i}},	\\
	h_{3}^{\text{dist}}\left(i,j,k,o_3|\bbeta_{\text{dist},3}\right) = \beta_{3,0}^{\text{dist}}	&	+ \beta_{3,1}^{\text{dist}}\lnf{d_{k,o_3}}	+ \beta_{3,2}^{\text{dist}}\lnf{d_{k,i}}	+ \beta_{3,3}^{\text{dist}}\lnf{d_{k,j}}	\\*
				&	+ \beta_{3,4}^{\text{dist}}\lnf{d_{o_3,i}}	+ \beta_{3,5}^{\text{dist}}\lnf{d_{o_3,j}},
\end{align*}
with
\begin{align*}
	\bbeta_{\text{dist},1}	&	= \left(\beta_{1,0}^{\text{dist}}, \beta_{1,1}^{\text{dist}}\right)\T \in \R^{2},	\\*
	\bbeta_{\text{dist},2}	&	= \left(\beta_{2,0}^{\text{dist}}, \ldots, \beta_{2,3}^{\text{dist}}\right)\T \in \R^{4},	\\*
	\bbeta_{\text{dist},3}	&	= \left(\beta_{3,0}^{\text{dist}}, \ldots, \beta_{3,5}^{\text{dist}}\right)\T \in \R^{6}.
\end{align*}
All possible distances are included. The occurring parameters are summarized as
\beqo
	\bbeta_{\text{dist}}^{\text{SCVM}} = \left(\bbeta_{\text{dist},1}\T,\bbeta_{\text{dist},2}\T,\bbeta_{\text{dist},3}\T\right)\T \in \R^{n_\text{par}^\text{dist}},
\eeqo
where $n_\text{par}^\text{dist} = 2+4+6 = 12$.

The \emph{d0 reparametrization} (d0) is defined by the model functions
\begin{align*}
	h_{1}^{\text{d0}}\left(i,o_1|\bbeta_{\text{d0},1}\right) &	= \beta_{1,0}^{\text{d0}}	+ \beta_{1,1}^{\text{d0}}\lnf{d_{i,o_1}},	\\
	h_{2}^{\text{d0}}\left(i,j,o_2|\bbeta_{\text{d0},2}\right) &	= \beta_{2,0}^{\text{d0}}	+ \beta_{2,1}^{\text{d0}}\lnf{d_{j,o_2}},	\\
	h_{3}^{\text{d0}}\left(i,j,k,o_3|\bbeta_{\text{d0},3}\right) &	= \beta_{3,0}^{\text{d0}}	+ \beta_{3,1}^{\text{d0}}\lnf{d_{k,o_3}},
\end{align*}
where
\begin{align*}
	\bbeta_{\text{d0},1}	&	= \left(\beta_{1,0}^{\text{d0}}, \beta_{1,1}^{\text{d0}}\right)\T \in \R^{2},	\\*
	\bbeta_{\text{d0},2}	&	= \left(\beta_{2,0}^{\text{d0}}, \beta_{2,1}^{\text{d0}}\right)\T \in \R^{2},	\\*
	\bbeta_{\text{d0},3}	&	= \left(\beta_{3,0}^{\text{d0}}, \beta_{3,1}^{\text{d0}}\right)\T \in \R^{2}.
\end{align*}
Only the distances indicated by the conditioned sets of the copulae are involved. The parameters of the d0 reparametrization are summarized as
\beqo
	\bbeta_{\text{d0}}^{\text{SCVM}} = \left(\bbeta_{\text{d0},1}\T,\bbeta_{\text{d0},2}\T,\bbeta_{\text{d0},3}\T\right)\T \in \R^{n_\text{par}^\text{d0}},
\eeqo
where $n_\text{par}^\text{d0} = 3\cdot2 = 6$.

Again we also consider reparametrizations called \emph{elevation reparametrization} (elev) and \emph{e0 reparametrization} (e0). They are obtained analogous to the distance and d0 reparametrization, by choosing elevation differences instead of distances.

Eventually the \emph{d0+e0 reparametrization} (de) is given by
\begin{align*}
	h_{1}^{\text{de}}\left(i,o_1|\bbeta_{\text{de},1}\right) = \beta_{1,0}^{\text{de}}	&	+ \beta_{1,1}^{\text{de}}\lnf{d_{i,o_1}} + \beta_{1,2}^{\text{de}}\lnf{e_{i,o_1}},	\\
	h_{2}^{\text{de}}\left(i,j,o_2|\bbeta_{\text{de},2}\right) = \beta_{2,0}^{\text{de}}	&	+ \beta_{2,1}^{\text{de}}\lnf{d_{j,o_2}} + \beta_{2,2}^{\text{de}}\lnf{e_{j,o_2}},	\\
	h_{3}^{\text{de}}\left(i,j,k,o_3|\bbeta_{\text{de},3}\right) = \beta_{3,0}^{\text{de}}	&	+ \beta_{3,1}^{\text{de}}\lnf{d_{k,o_3}} + \beta_{3,2}^{\text{de}}\lnf{e_{k,o_3}},
\end{align*}
and
\begin{align*}
	\bbeta_{\text{de},1}	&	= \left(\beta_{1,0}^{\text{de}}, \beta_{1,1}^{\text{de}}, \beta_{1,2}^{\text{de}}\right)\T \in \R^{3},	\\*
	\bbeta_{\text{de},2}	&	= \left(\beta_{2,0}^{\text{de}}, \beta_{2,1}^{\text{de}}, \beta_{2,2}^{\text{de}}\right)\T \in \R^{3},	\\*
	\bbeta_{\text{de},3}	&	= \left(\beta_{3,0}^{\text{de}}, \beta_{3,1}^{\text{de}}, \beta_{3,2}^{\text{de}}\right)\T \in \R^{3}.
\end{align*}
It involves the distances and elevation differences indicated by the respective conditioned sets. The summary of its parameters is given by
\beqo
	\bbeta_{\text{de}}^{\text{SCVM}} = \left(\bbeta_{\text{de},1}\T,\bbeta_{\text{de},2}\T,\bbeta_{\text{de},3}\T\right)\T \in \R^{n_\text{par}^\text{de}}
\eeqo
where $n_\text{par}^\text{de} = 3\cdot3 = 9$.

In order to terminate the reparametrization of the composite vine model parameters, a reparametrization of the second copula parameters respectively the degrees of freedom $\bnu^{\text{CVM}}$ is required. As before, we investigate the parameters stemming from the composite vine model on the mean temperature data.

Let $\wh\nu_{ij|\ldots}$ denote any arbitrary degrees of freedom parameter of our composite vine model, irrespective of the tree which the parameter stems from. Figure \ref{fig:SCVM:nu} shows plots of the parameters $\wh\nu_{ij|\ldots}$ against their respective tree number and against the distances $d_{i,j}$ and elevation differences $e_{i,j}$. % corresponding to the variable pairs $\{i,j\}$ constituting the conditio_1ned sets of the edges corresponding to the parameters $\wh\nu_{ij|\calD}$.
From the plots we observe, that the average degrees of freedom rise with the tree number. Moreover there seems to be a significant trend of the parameters $\wh\nu_{ij|\ldots}$ with respect to the distances $d_{i,j}$, but there is no evident influence of the elevation differences.

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{Figures/SpatialCompTDE04.pdf}
	\caption[Plots of $\wh\nu_{ij|...}$ against tree number, $\ln(d_{i,j})$ and $\ln(e_{i,j})$, respectively.]{Plots of $\wh\nu_{ij|...}$ against tree number, $\ln(d_{i,j})$ and $\ln(e_{i,j})$, respectively.}
	\label{fig:SCVM:nu}
\end{figure}

Due to our observations on Figure \ref{fig:SCVM:nu}, we are going to use the reparametrization
\begin{align}\label{eq:SCVM:nu}
	\wt\nu_{io_1}	&	= \exp\left(\beta_{0}^{\nu} + \beta_{1}^{\nu}\cdot1 + \beta_{2}^{\nu}d_{i,o_1}\right),	\nonumber\\*
	\wt\nu_{jo_2|i}	&	= \exp\left(\beta_{0}^{\nu} + \beta_{1}^{\nu}\cdot2 + \beta_{2}^{\nu}d_{j,o_2}\right),	\\*
	\wt\nu_{ko_3|ij}	&	= \exp\left(\beta_{0}^{\nu} + \beta_{1}^{\nu}\cdot3 + \beta_{2}^{\nu}d_{k,o_3}\right),	\nonumber
\end{align}
of the second copula parameters. The respective parameters are summarized as
\beqo
	\bbeta_{\nu}^{\text{SCVM}} = \left(\beta_{0}^{\nu},\beta_{1}^{\nu},\beta_{2}^{\nu}\right)\T \in \R^{n_\text{par}^\nu},
\eeqo
where $n_\text{par}^\nu= 3$.


A (three neighbors) composite vine model which is reparametrized by reparametrizations of the type \eqref{eq:SCVM:repar} and \eqref{eq:SCVM:nu}, will be called (three neighbors) \emph{spatial composite vine model (SCVM)}. In order to estimate the respective model parameters, the composite log-likelihood \eqref{eq:compll} parametrized via \eqref{eq:SCVM:repar} and \eqref{eq:SCVM:nu} has to be maximized. This yields the maximum composite likelihood estimates (mcle)
\beqo
	\wh\bbeta_{\text{mcle}}^{\text{SCVM}} = \left(\wh\bbeta_{\text{mod}}^{\text{SCVM}}, \wh\bbeta_\nu^{\text{SCVM}}\right)\T \in \R^{(n_\text{par}^\text{mod}+n_\text{par}^\nu)}.
\eeqo

From now on, we will address the above specified spatial composite vine models according to the selected reparametrization as full, distance, d0, elevation, e0 or d0+e0 model.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Section 05 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A spatial composite vine model for mean temperature}\label{sec:SCVM:app}

This application of the previously specified model is intended to investigate a spatial composite vine model for the mean temperature data set. For this purpose we are going to choose a suitable reparametrization of the composite vine model which was set up in Subsection \ref{sec:CVM:app}.


\subsubsection{Model selection}\label{sec:app:SCVMselect}

Table \ref{tab:SCVM:npar} summarizes the required number of parameters for the six models specified up to now. Even the full model needs only $24$ parameters. We will conduct further analyses in the following, intended to check, if the number of parameters can be reduced even more.

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Sat Jun 29 23:27:28 2013
\begin{table}[htb]
\centering
\begin{tabular}{l|rrrrrr}
	 & full & distance & d0 & elevation & e0 & d0+e0 \\
  \hline
  \hline
	Tree 1 & 3 & 2 & 2 & 2 & 2 & 3 \\ 
  Tree 2 & 7 & 4 & 2 & 4 & 2 & 3 \\ 
  Tree 3 & 11 & 6 & 2 & 6 & 2 & 3 \\ 
  $n_\text{par}^\nu$ & 3 & 3 & 3 & 3 & 3 & 3 \\ 
	\hline
  \textbf{Sum} & \textbf{24} & \textbf{15} & \textbf{9} & \textbf{15} & \textbf{9} & \textbf{12} \\ 
\end{tabular}
\caption[Number of parameters for the 'full', 'distance', 'd0', 'elevation', 'e0' and 'd0+e0' model.]{Number of parameters for the 'full', 'distance', 'd0', 'elevation', 'e0' and 'd0+e0' model.} 
\label{tab:SCVM:npar}
\end{table}

In order to get a clue about the explanatory power of the six reparametrizations of the first copula parameters given in Section \ref{sec:SCVM}, we investigate the following linear models. For all reparametrizations (mod) among the reparametrizations (full), (dist), (d0), (elev), (e0), and (de), we define the linear models
	\begin{align*}
		\text{F}_z(\tau_{so})	&	= h_{1}^{\text{mod}}(s,o|\bbeta_{\text{mod},1}) + \veps_{so}, \quad \veps_{so}\simiid\vN{0}{\sigma^2},\quad o\in\{p_s,q_s,r_s\},	\\*
		\text{F}_z(\tau_{p_so|s})	&	= h_{2}^{\text{mod}}(s,p_s,o|\bbeta_{\text{mod},2}) + \veps_{p_so|s}, \quad \veps_{p_so|s}\simiid\vN{0}{\sigma^2},\quad o\in\{q_s,r_s\},	\\*
		\text{F}_z(\tau_{q_sr_s|sp_s})	&	= h_{3}^{\text{mod}}(s,p_s,q_s,r_s|\bbeta_{\text{mod},3}) + \veps_{q_sr_s|sp_s}, \quad \veps_{q_sr_s|sp_s}\simiid\vN{0}{\sigma^2},
	\end{align*}
where $\iN{s}{54}$. The $\Rsq$ and $\Rsqa$ which are obtained from fitting these linear modes are summarized in Table \ref{tab:SCVM:R2}. The resulting parameter estimates can be used as start parameters for $\bbeta_{\text{mod}}$ for the purpose of fitting a spatial composite vine model on the mean temperature data set.

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Sat Jun 29 23:27:28 2013
\begin{table}[htb]
\centering
\footnotesize
\begin{tabular}{l|llllll}
	Tree & full & distance & d0 & elevation & e0 & d0+e0 \\ 
  \hline
  \hline
	1 & 0.579 (0.574) & 0.487 (0.484) & 0.487 (0.484) & 0.098 (0.092) & 0.098 (0.092) & 0.579 (0.574) \\ 
  2 & 0.735 (0.719) & 0.718 (0.710) & 0.455 (0.450) & 0.071 (0.045) & 0.006 (-0.004) & 0.457 (0.446) \\ 
  3 & 0.811 (0.767) & 0.780 (0.758) & 0.633 (0.626) & 0.183 (0.098) & 0.036 (0.017) & 0.634 (0.620) \\ 
\end{tabular}
\caption[$\Rsq$ (and $\Rsqa$) for the 'full', 'distance', 'd0', 'elevation', 'e0' and 'd0+e0' model.]{$\Rsq$ (and $\Rsqa$) for the 'full', 'distance', 'd0', 'elevation', 'e0' and 'd0+e0' model.} 
\label{tab:SCVM:R2}
\end{table}

%% latex table generated in R 2.15.0 by xtable 1.7-1 package
%% Sat Jun 29 23:27:28 2013
%\begin{table}[htb]
%\centering
%\begin{tabular}{l|rrrrrr}
%	Tree & full & distance & d0 & elevation & e0 & d0+e0 \\ 
%  \hline
%  \hline
%	1 & 0.5736 & 0.4841 & 0.4841 & 0.0924 & 0.0924 & 0.5736 \\ 
%  2 & 0.7191 & 0.7102 & 0.4497 & 0.0447 & -0.0035 & 0.4462 \\ 
%  3 & 0.7667 & 0.7575 & 0.6264 & 0.0983 & 0.0171 & 0.6198 \\ 
%\end{tabular}
%\caption[$\Rsqa$ for the 'full', 'distance', 'd0', 'elevation', 'e0' and 'd0+e0' model.]{$\Rsqa$ for the 'full', 'distance', 'd0', 'elevation', 'e0' and 'd0+e0' model.} 
%\label{tab:SCVM:adjR2}
%\end{table}

Comparison of the values given in Table \ref{tab:SCVM:R2} again yields bad performance of the elevation and e0 model, which include only elevation differences. For the first trees the d0+e0 respectively the full model is distinctly superior compared to the other models. Considering the $\Rsqa$ for the second and third trees, the d0 model outperforms the d0+e0 model. Extension of the d0 model to the distance model yields a considerable improvement in terms of the $\Rsq$, respectively $\Rsqa$. Since the distance model performs similarly well as the full model for the trees two and three, we decide to choose a mixed reparametrization (select) of the first copula parameters, which is build up of the (de) reparametrization for the first trees and the (dist) reparametrization for the second and third trees.

The model functions $h_{l}^{\text{select}}$, $l=1,2,3$, of the reparametrization (select) are given as
\begin{align}\label{eq:select}
	h_{1}^{\text{select}}\left(i,o_1|\bbeta_{\text{select},1}\right)	&	= h_{1}^{\text{de}}\left(i,o_1|\bbeta_{\text{select},1}\right),	\nonumber	\\
	h_{2}^{\text{select}}\left(i,j,o_2|\bbeta_{\text{select},2}\right)	&	= h_{2}^{\text{dist}}\left(i,j,o_2|\bbeta_{\text{select},2}\right),	\\
	h_{3}^{\text{select}}\left(i,j,k,o_3|\bbeta_{\text{select},3}\right)	&	= h_{3}^{\text{dist}}\left(i,j,k,o_3|\bbeta_{\text{select},3}\right),	\nonumber
\end{align}
where
\begin{align*}
	\bbeta_{\text{select},1}	&	= \left(\beta_{1,0}^{\text{select}}, \beta_{1,1}^{\text{select}}, \beta_{1,2}^{\text{select}}\right)\T \in \R^{3},	\\*
	\bbeta_{\text{select},2}	&	= \left(\beta_{2,0}^{\text{select}}, \ldots, \beta_{2,3}^{\text{select}}\right)\T \in \R^{4},	\\*
	\bbeta_{\text{select},3}	&	= \left(\beta_{3,0}^{\text{select}}, \ldots, \beta_{3,5}^{\text{select}}\right)\T \in \R^{6}.
\end{align*}
Its parameters are summarized as
\beqo
	\bbeta_{\text{select}}^{\text{SCVM}} = \left(\bbeta_{\text{select},1}\T,\bbeta_{\text{select},2}\T,\bbeta_{\text{select},3}\T\right)\T \in \R^{n_\text{par}^\text{select}},
\eeqo
where $n_\text{par}^\text{select} = 3+4+6 = 13$.

It remains to analyze the reparametrization \eqref{eq:SCVM:nu} of the second copula parameters. To this end we fit the linear model defined by
\begin{align*}
	\ln(\nu_{so})	&	= \beta_{0}^{\nu} + \beta_{1}^{\nu} \cdot 1 + \beta_{2}^{\nu}d_{s,o} + \veps_{so},	\quad o\in\{p_s,q_s,r_s\},	\\*
	\ln(\nu_{p_so|s})	&	= \beta_{0}^{\nu} + \beta_{1}^{\nu} \cdot 2 + \beta_{2}^{\nu}d_{p_s,o} + \veps_{p_so|s}, \quad o\in\{q_s,r_s\},	\\*
	\ln(\nu_{q_so|sp_s})	&	= \beta_{0}^{\nu} + \beta_{1}^{\nu} \cdot 3 + \beta_{2}^{\nu}d_{q_s,o} + \veps_{q_so|sp_s}, \quad o\in\{r_s\},
\end{align*}
where $\iN{s}{54}$ and $\veps_{sp_s}$, $\veps_{sq_s}$, $\veps_{sr_s}$, $\veps_{p_sq_s|s}$, $\veps_{p_sr_s|s}$, $\veps_{q_sr_s|sp_s}\simiid\vN{0}{\sigma^2}$ for $\iN{s}{54}$. The respective parameter estimates, their standard errors, Wald statistics and p-values are given in Table \ref{tab:SCVM:nu}. The estimates for $\beta_{0}^{\nu}$, $\beta_{1}^{\nu}$ and $\beta_{2}^{\nu}$ are significant at a significance level $\alpha=5\%$. %The one for $\beta_{0}^{\nu}$ scarcely misses significance.
These findings yield that the reparametrization \eqref{eq:SCVM:nu} is adequate for our purposes. As before, the obtained parameter estimates can be used as start values for $\bbeta_{\nu}$ within the framework of model fitting.

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Sat Jun 29 23:27:28 2013
\begin{table}[htb]
\centering
\begin{tabular}{l|rrrr}
 & Estimate & Std. Error & t-value & p-value \\ 
  \hline
	\hline
	$\beta_{0}^{\nu}$ & 0.6745 & 0.2900 & 2.33 & 0.0207 \\ 
  $\beta_{1}^{\nu}$ & 0.1532 & 0.0299 & 5.13 & 0.0000 \\ 
  $\beta_{2}^{\nu}$ & 0.2571 & 0.0677 & 3.80 & 0.0002 \\ 
\end{tabular}
\caption[Parameter estimates of the model for the second parameters $\nu_{ij}$.]{Parameter estimates, estimated standard errors, Wald statistics and p-values of the model for the second parameters $\nu_{ij}$.} 
\label{tab:SCVM:nu}
\end{table}

All in all we have selected a reparametrization according to \eqref{eq:select} and \eqref{eq:SCVM:nu}, which is based on $n_\text{par}^\text{select} + n_\text{par}^\nu = 16$ parameters. In the following we will call the resulting model \emph{selected spatial composite vine model.} %The next subsubsection treats the maximum composite likelihood estimation of the model parameters.




\subsubsection{Model fit}\label{sec:app:SCVMfit}

Next we are going to fit our selected spatial composite vine model to the data. This is conducted by maximization of the composite log-likelihood \eqref{eq:compll} which is reparametrized by means of \eqref{eq:select} and \eqref{eq:SCVM:nu}. This time we get a maximum composite log-likelihood of $\cll{\text{SCVM}}{\wh\bbeta_\text{select}^{\text{SCVM}}, \wh\bbeta_\nu^{\text{SCVM}}}{\bu^1,\ldots,\bu^d}=40938.80$, AIC and BIC are given as $\AIC_\text{SCVM}=-81845.6$ and $\BIC_\text{SCVM}=-81765.7$. Compared to the composite vine model the composite log-likelihood of the spatial composite vine model shrinked by about $1168$. Due to the fact that the number of parameters is reduced considerably, the BIC of the spatial composite vine model is smaller. Comparison based on the AIC would however favor the composite vine model. 

The fitting procedure yields the parameter estimates $\wh\bbeta_{\text{mcle}}^{\text{SCVM}} \coloneqq (\wh\bbeta_{\text{select}}^{\text{SCVM}}, \wh\bbeta_\nu^{\text{SCVM}})\T \in \R^{16}$, which are given in Table \ref{tab:SCVMmcle}. The table moreover compares the parameter estimates to their respective start values, which were already addressed in the previous subsection.

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Tue Jul 16 21:45:17 2013
\begin{table}[htb]
\centering
\begin{tabular}{rlrr|rlrr|rlrr}
	no. & par & start & mcle & no. & par & start & mcle & no. & par & start & mcle \\ 
  \hline
	\hline
	1 & $\beta_{1,0}^\text{select}$ & 2.300 & 2.251 & 7 & $\beta_{2,3}^\text{select}$ & 0.297 & 0.248 & 13 & $\beta_{3,5}^\text{select}$ & 0.120 & 0.119 \\ 
  2 & $\beta_{1,1}^\text{select}$ & -0.305 & -0.299 & 8 & $\beta_{3,0}^\text{select}$ & 0.256 & 0.704 & 14 & $\beta_0^\nu$ & 0.675 & 0.404 \\ 
  3 & $\beta_{1,2}^\text{select}$ & -0.025 & -0.022 & 9 & $\beta_{3,1}^\text{select}$ & -0.434 & -0.405 & 15 & $\beta_1^\nu$ & 0.153 & 0.015 \\ 
  4 & $\beta_{2,0}^\text{select}$ & 0.306 & 0.577 & 10 & $\beta_{3,2}^\text{select}$ & 0.109 & 0.076 & 16 & $\beta_2^\nu$ & 0.257 & 0.271 \\ 
  5 & $\beta_{2,1}^\text{select}$ & -0.510 & -0.480 & 11 & $\beta_{3,3}^\text{select}$ & 0.089 & 0.016 &  &  &  &  \\ 
  6 & $\beta_{2,2}^\text{select}$ & 0.222 & 0.175 & 12 & $\beta_{3,4}^\text{select}$ & 0.115 & 0.095 &  &  &  &  \\ 
\end{tabular}
\caption[Start values and maximum composite-likelihood estimates of the spatial composite vine model for the mean temperature data.]{Start values and maximum composite-likelihood estimates of the spatial composite vine model for the mean temperature data.} 
\label{tab:SCVMmcle}
\end{table}


\subsubsection{Prediction}\label{sec:app:SCVMpred}

Again we aim to predict from our newly developed model. The structure of the spatial composite vine model suggests to perform prediction based on a four-dimensional C-vine which is composed out of the variables corresponding to the new location $s$ from which to predict and to its three closest neighbors among the stations $1,\ldots,d$. As before we denote the closest observation station as $p_s$, the second closest neighbor as $q_s$ and the third closest station as $r_s$.
%\beqo
	%\wh u_s = F_{s|p_sq_sr_s}^{-1}(v_s|u_{p_s},u_{q_s},u_{r_s}), \quad \mbox{for } v_s\sim\vU01
%\eeqo
%The values of $u_{p_s}$, $u_{q_s}$ and $u_{r_s}$ are known (training data set on which the model is built).

For the purpose of prediction we are going to sample from the conditional distribution $F_{s|p_sq_sr_s}(u^s|u^{p_s},u^{q_s},u^{r_s})$. It has to be calculated iteratively according to Lemma \ref{lem:transvar}. Based on the copulae needed for these calculations, we are going to set up the corresponding C-vine. For convenience we drop the arguments of the conditional distribution functions $F$ in the following, since it is anyway indicated in the indices which arguments to use. Moreover the estimates of the first and the second copula parameters, whose calculation will be presented later on, are denoted by $\wh\theta$ and $\wh\nu$, respectively, the corresponding copula families are denoted by $t$ with respective indices.

The conditional distribution $F_{s|p_sq_sr_s}$ is calculated as
\beqo
	F_{s|p_sq_sr_s}	=	\frac{\partial \Cop{r_ss;p_sq_s}{F_{s|p_sq_s},F_{r_s|p_sq_s}\sepi\wh\te_{r_ss|p_sq_s},\wh\nu_{r_ss|p_sq_s},t_{r_ss|p_sq_s}}}{\partial F_{r_s|p_sq_s}}.
\eeqo
This yields that we are going to use $r_ss|p_sq_s$ as edge for the third C-vine tree. The iteration continues with the two equations
\beqo
	F_{r_s|p_sq_s} = \frac{\partial \Cop{q_sr_s;p_s}{F_{r_s|p_s},F_{q_s|p_s}\sepi\wh\te_{q_sr_s|p_s},\wh\nu_{q_sr_s|p_s},t_{q_sr_s|p_s}}}{\partial F_{q_s|p_s}},
\eeqo
and
\beqo
	F_{s|p_sq_s} = \frac{\partial \Cop{q_ss;p_s}{F_{s|p_s},F_{q_s|p_s}\sepi\wh\te_{q_ss|p_s},\wh\nu_{q_ss|p_s},t_{q_ss|p_s}}}{\partial F_{q_s|p_s}},
\eeqo
which yields the second tree edges $q_sr_s|p_s$ and $q_ss|p_s$. The arguments needed above are furthermore calculated via
\begin{align*}
	F_{q_s|p_s} & = \frac{\partial \Cop{p_sq_s}{F_{q_s},F_{p_s}\sepi\wh\te_{p_sq_s},\wh\nu_{p_sq_s},t_{p_sq_s}}}{\partial F_{p_s}}	=	\frac{\partial \Cop{p_sq_s}{u^{q_s},u^{p_s}\sepi\wh\te_{p_sq_s},\wh\nu_{p_sq_s},t_{p_sq_s}}}{\partial u^{p_s}},	\\
	F_{r_s|p_s} & = \frac{\partial \Cop{p_sr_s}{F_{r_s},F_{p_s}\sepi\wh\te_{p_sr_s},\wh\nu_{p_sr_s},t_{p_sr_s}}}{\partial F_{p_s}}	=	\frac{\partial \Cop{p_sr_s}{u^{r_s},u^{p_s}\sepi\wh\te_{p_sr_s},\wh\nu_{p_sr_s},t_{p_sr_s}}}{\partial u^{p_s}},	\\
	F_{s|p_s} & = \frac{\partial \Cop{p_ss}{F_{s} ,F_{p_s} \sepi\wh\te_{p_ss},\wh\nu_{p_ss},t_{p_ss}}}{\partial F_{p_s} }	=	\frac{\partial \Cop{p_ss}{u^{s},u^{p_s}\sepi\wh\te_{p_ss},\wh\nu_{p_ss},t_{p_ss}}}{\partial u^{p_s}}.
\end{align*}
The unconditioned distributions $F_{s}$, $F_{p_s}$, $F_{q_s}$, $F_{r_s}$ involved here are known to be the cumulative distribution functions of $\vU01$ distributed random variables. Following it holds that $F_{o}(u^o)=u^o$ for $o\in\{s,p_s,q_s,r_s\}$. We gain $p_sq_s$, $p_sr_s$ and $p_ss$ for the three edges of the first C-vine tree. All in all we obtain the C-vine illustrated in Figure \ref{fig:pred:cvine}.

%\begin{figure}[htb]
	%\centerline{
		%\entrymodifiers={++[o][F]}
		%%\SelectTips{cm}{}
		%\xymatrix @+2pc {
		%*{\tree_1}					& *\txt{}										&	*{\tree_2}									& *\txt{}													&	*{\tree_3}							\\
		%p_s									& q_s \ar@{-}[l]_{p_sq_s}		&	p_sq_s											& *\txt{}													& q_sr_s|p_s \ar@{-}[d]^{r_ss|p_sq_s}	\\
		%s	\ar@{-}[u]_{p_ss}	& r_s \ar@{-}[ul]_{p_sr_s}	&	p_ss \ar@{-}[u]_{q_ss|p_s}	& p_sr_s \ar@{-}[ul]_{q_sr_s|p_s}	& q_ss|p_s										\\
		%}
	%}
	%\caption{C-vine structure in order to sample from $F_{s|p_sq_sr_s}(u^s|u^{p_s},u^{q_s},u^{r_s})$.}
	%\label{fig:pred:cvine}
%\end{figure}

\begin{figure}[htb]
	\centerline{
		\entrymodifiers={++[o][F]}
		%\SelectTips{cm}{}
		\xymatrix @+2pc {
		p_s									& q_s \ar@{-}[l]_{p_sq_s}		&	p_sq_s											& *\txt{}													& q_sr_s|p_s \ar@{-}[d]^{r_ss|p_sq_s}	\\
		s	\ar@{-}[u]_{p_ss}	& r_s \ar@{-}[ul]_{p_sr_s}	&	p_ss \ar@{-}[u]_{q_ss|p_s}	& p_sr_s \ar@{-}[ul]_{q_sr_s|p_s}	& q_ss|p_s										\\
		}
	}
	\caption{C-vine structure in order to sample from $F_{s|p_sq_sr_s}(u^s|u^{p_s},u^{q_s},u^{r_s})$.}
	\label{fig:pred:cvine}
\end{figure}

In order to be able to simulate from $F_{s|p_sq_sr_s}(u^s|u^{p_s},u^{q_s},u^{r_s})$, we have to specify the copula families and the respective parameters involved in the calculations above. The first copula parameters are calculated based on the model functions of the selected spatial composite vine model and the respective parameter estimates according to
\begin{align*}
	\wh\te_{p_sq_s}	&	=	\itau\left(\Fzi \left(h_{1}^{\text{select}}\left(p_s,q_s|\wh\bbeta_{\text{select},1}\right)\right); t_{p_sq_s}\right),	\\
	\wh\te_{p_sr_s}	&	=	\itau\left(\Fzi \left(h_{1}^{\text{select}}\left(p_s,r_s|\wh\bbeta_{\text{select},1}\right)\right); t_{p_sr_s}\right),	\\
	\wh\te_{p_ss}	&	=	\itau\left(\Fzi \left(h_{1}^{\text{select}}\left(p_s,s|\wh\bbeta_{\text{select},1}\right)\right); t_{p_ss}\right),	\\
	\wh\te_{q_sr_s|p_s}	&	=	\itau\left(\Fzi \left(h_{2}^{\text{select}}\left(p_s,q_s,r_s|\wh\bbeta_{\text{select},2}\right)\right); t_{q_sr_s|p_s}\right),	\\
	\wh\te_{q_ss|p_s}	&	=	\itau\left(\Fzi \left(h_{2}^{\text{select}}\left(p_s,q_s,s|\wh\bbeta_{\text{select},2}\right)\right); t_{q_ss|p_s}\right),	\\
	\wh\te_{r_ss|p_sq_s}	&	=	\itau\left(\Fzi \left(h_{3}^{\text{select}}\left(p_s,q_s,r_s,s|\wh\bbeta_{\text{select},3}\right)\right); t_{r_ss|p_sq_s}\right),
\end{align*}
where $t_{p_sq_s}$, $t_{p_sr_s}$, $t_{p_ss}$, $t_{q_sr_s|p_s}$, $t_{q_ss|p_s}$ and $t_{r_ss|p_sq_s}$ denote the respective copula families. Due to the fact that most copulae in our selected spatial composite vine model were determined to be Student-$t$ copulae (see Table \ref{tab:CVM:fam}), we choose the Student-$t$ family for all of these families. Following we have to determine a second copula parameter for each of the six Student-$t$ copulae involved. According to the reparametrization \eqref{eq:SCVM:nu}, we obtain
\begin{align*}
	\wh\nu_{p_sq_s}	&	= \exp\left(\wh\beta_{0}^{\nu} + \wh\beta_{1}^{\nu} + \wh\beta_{2}^{\nu}d_{p_s,q_s}\right),	\\
	\wh\nu_{p_sr_s}	&	= \exp\left(\wh\beta_{0}^{\nu} + \wh\beta_{1}^{\nu} + \wh\beta_{2}^{\nu}d_{p_s,r_s}\right),	\\
	\wh\nu_{p_ss}	&	= \exp\left(\wh\beta_{0}^{\nu} + \wh\beta_{1}^{\nu} + \wh\beta_{2}^{\nu}d_{p_s,s}\right),	\\
	\wh\nu_{q_sr_s|p_s}	&	= \exp\left(\wh\beta_{0}^{\nu} + 2\wh\beta_{1}^{\nu} + \wh\beta_{2}^{\nu}d_{q_s,r_s}\right),	\\
	\wh\nu_{q_ss|p_s}	&	= \exp\left(\wh\beta_{0}^{\nu} + 2\wh\beta_{1}^{\nu} + \wh\beta_{2}^{\nu}d_{q_s,s}\right),	\\
	\wh\nu_{r_ss|p_sq_s}	&	= \exp\left(\wh\beta_{0}^{\nu} + 3\wh\beta_{1}^{\nu} + \wh\beta_{2}^{\nu}d_{r_s,s}\right).
\end{align*}

Furthermore we are interested in the predictive density $f_{s|p_sq_sr_s}$ corresponding to $F_{s|p_sq_sr_s}$. It is calculated similarly to the conditioned R-vine density in Subsection \ref{sec:app:SVpred} of Section \ref{sec:svines}. We obtain
\begin{align}\label{eq:SCVMpdist}
	f_{s|p_sq_sr_s}	&	= \cop{p_ss}{F_{p_s},F_{s}\sepi\wh\te_{p_ss},\wh\nu_{p_ss},t_{p_ss}}	\nonumber	\\*	
		&	\cdot	\cop{q_ss;p_s}{F_{q_s|p_s},F_{s|p_s}\sepi\wh\te_{q_ss|p_s},\wh\nu_{q_ss|p_s},t_{q_ss|p_s}}	\\*
		&	\cdot	\cop{r_ss;p_sq_s}{F_{r_s|p_sq_s},F_{s|p_sq_s}\sepi\wh\te_{r_ss|p_sq_s},\wh\nu_{r_ss|p_sq_s},t_{r_ss|p_sq_s}}.	\nonumber
\end{align}

This concludes the methodology of prediction from spatial composite R-vine models on the copula data level. The copula data obtained from the simulations can be transformed back to the original data level as described in Subsection \ref{sec:app:SVpred} of the previous section.

The results of the spatial composite R-vine model based predictions of the mean temperatures at the $24$ observation stations constituting the validation data set are visualized in Figures \ref{fig:SCVMpred01}-\ref{fig:SCVMpredbox04}. Since they show the results of the predictions in analogy to Figures \ref{fig:SVpred01}-\ref{fig:SVpredbox04} and due to the fact that the results are pretty similar, however not identical, we do not discuss every figure in detail and refer instead to the observations of Subsection \ref{sec:app:SVpred} in Section \ref{sec:svines}. The respective plots for the three selected stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$) are given by Figures \ref{fig:SCVMpredMSE}-\ref{fig:SCVMpredresMSE}.

We again summarize the mean squared prediction errors in Table \ref{tab:SCVM:MSE}. As before \emph{Arkona} ($57$) has an outstanding high mean squared error among the stations with elevations smaller than $500$ meters. The reason why we have problems with the prediction of mean temperatures at Arkona may originate from the location of the observation station. Due to the fact that the observation station Arkona lies on an island in the Baltic Sea, it has an outstanding position compared to the rest of our observation stations and it may be exposed to factors which are not captured by our models. Once again the mean squared errors and the plots for the observation stations \emph{Neuhaus am Rennweg} ($75$) and \textit{Großer Arber} ($69$) show obviously that the prediction fails in these cases.

% latex table generated in R 2.15.0 by xtable 1.7-1 package
% Mon Jul 29 18:30:38 2013
\begin{table}[htb]
\centering
\begin{tabular}{rlrr|rlrr}
	s & short name & elevation & $\text{MSE}(s)$ & s & short name & elevation & $\text{MSE}(s)$ \\ 
  \hline
	\hline
	61 & \texttt{bork} & 3.00 & 0.55 &   63 & \texttt{buch} & 340.00 & 1.21 \\ 
  62 & \texttt{bvoe} & 10.00 & 0.38 &  65 & \texttt{ebra} & 346.00 & 0.92 \\ 
  72 & \texttt{luec} & 17.00 & 0.30 &  60 & \texttt{blan} & 417.00 & 0.66 \\ 
  68 & \texttt{gram} & 27.00 & 0.22 &  66 & \texttt{ellw} & 460.00 & 0.90 \\ 
  64 & \texttt{cosc} & 40.00 & 0.92 &  59 & \texttt{augs} & 461.40 & 0.47 \\ 
  57 & \texttt{arko} & 42.00 & 2.32 &  67 & \texttt{falk} & 472.00 & 0.41 \\ 
  77 & \texttt{rahd} & 42.00 & 0.25 &  76 & \texttt{ohrz} & 494.00 & 0.72 \\ 
  70 & \texttt{grue} & 55.90 & 0.19 &  71 & \texttt{hohe} & 743.30 & 3.42 \\ 
  56 & \texttt{alfe} & 143.90 & 0.23 &  55 & \texttt{albs} & 759.00 & 2.04 \\ 
  58 & \texttt{arns} & 159.00 & 0.98 &  75 & \texttt{neuh} & 845.00 & 6.45 \\ 
  78 & \texttt{wies} & 187.00 & 0.99 &  73 & \texttt{mitt} & 981.00 & 2.90 \\ 
  74 & \texttt{muel} & 273.00 & 0.68 &  69 & \texttt{garb} & 1436.00 & 15.07 \\ 
\end{tabular}
\caption[Mean squared errors for the observation stations of the validation data set (spatial composite vine model).]{Mean squared errors of the mean temperature predictions over the period 01/01/2010-12/31/2012 for the observation stations of the validation data set based on the spatial composite vine model.} 
\label{tab:SCVM:MSE}
\end{table}

Whereas the mean squared errors given in the Tables \ref{tab:SV:MSE} and \ref{tab:SCVM:MSE} allow a first comparison of the different prediction methods respectively models, we are going to perform an extensive model comparison in the following section, which is amongst others based on scoring.

\begin{landscape}
\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.30\textwidth]{Figures/SCVMpredMSE.pdf}
	\caption[Prediction of the mean temperatures for the observation stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$) based on the spatial composite vine model.]{Prediction of the mean temperatures for the observation stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$) for the period 01/01/2010-12/31/2012 based on the spatial composite vine model. black line: observed values. dark gray line: prediction. light gray area: $95\%$ prediction intervals.}
	\label{fig:SCVMpredMSE}
\end{figure}
\end{landscape}

\begin{landscape}
\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.30\textwidth]{Figures/SCVMpredresMSE.pdf}
	\caption[Prediction errors of the predictions for the observation stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$) based on the spatial composite vine model.]{Prediction errors of the predictions for the observation stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$) for the period 01/01/2010-12/31/2012 based on the spatial composite vine model.}
	\label{fig:SCVMpredresMSE}
\end{figure}
\end{landscape}

%\begin{landscape}
%\begin{figure}[htbp]
%	\centering
%		\includegraphics[width=1.20\textwidth]{Figures/SCVMpredbox2MSE.pdf}
%	\caption[$95\%$ prediction intervals, point predictions and observed mean temperatures for the first days of each months during the years $2010$-$2012$ for the observation stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$), based on the predictive distribution of the respective observation station (spatial composite vine model).]{$95\%$ prediction intervals, point predictions and observed mean temperatures for the first days of each months during the years $2010$-$2012$ for the observation stations Grünow ($70$), Arkona ($57$) and Großer Arber ($69$), each calculated based on $1000$ simulations from the predictive distribution of the mean temperatures at the respective observation station (spatial composite vine model).}
%	\label{fig:SCVMpredboxMSE}
%\end{figure}
%\end{landscape}

\cleardoublepage


==> Sections/Conclusions.tex <==

\section[Conclusions and outlook]{Conclusions and outlook}\label{sec:conc}

Finally we aim to summarize the results of the investigations performed in this thesis and give a brief outlook on possible model improvements and future fields of interest. The modeling process in this thesis evolved starting from a marginal model to the presentation of two new vine copula based models for spatial dependencies, the spatial R-vine model and the spatial composite vine model, and ended in an evaluation and comparison of these models. Furthermore, prediction methods based on the presented models were introduced. The fundament of all modeling was a data set of daily mean temperatures at $54$ selected observation stations across Germany.

The marginal model is intended to capture the marginal trends and distributions of the single variables whose dependencies are modeled subsequently. Besides an intercept term, components which capture the seasonal fluctuations and the temporal dependencies of the data are included into the regression model of the marginals. Moreover we found that a skew-$t$ distribution is an appropriate distribution for the error terms of the regression model, since we observed a skew and heavy tails for the residuals calculated from the data. Due to the fact that the final goal of the thesis is the prediction from the developed models, it was reasonable to model all marginals jointly, depending on elevation, longitude and latitude. An investigation of the parameter estimates obtained from separate marginal model fits led to the replacement of the model parameters by polynomials of these quantities. Further investigations showed, that the eventually developed marginal model, which is summarized in the subsequent box, is able to eliminate any seasonal fluctuations and time dependencies in the data to a reasonable extent. However we found that our marginal model can lead to inadequate prediction results if the location from which to predict lies outside the range of the data based on which we developed our models. Obviously, this is due to the inclusion of the polynomial components into our model. As already addressed in Chapter \ref{sec:svines}, there is room for an improvement of our marginal model, for instance by applying B-splines instead of the polynomials. On the other hand it might be reasonable to select the training data observation stations such that their locations are evenly spread over the area from which one wants to predict.

\noindent\fbox{\parbox[l]{0.985\textwidth}{
\noindent\textbf{joint marginal model (JMM):}\\
\begin{align*}
	\wt Y_t^s & = g\left(t, \wt Y_{t-1}^s, \wt Y_{t-2}^s, \wt Y_{t-3}^s, x_{\text{elev},s}, x_{\text{long},s}, x_{\text{lat},s} \sepi \bbeta_\text{ls}\right) + \veps_t^s	\\*
	\veps_t^s & \sim \vst{\xi(s)}{\omega(s)}{\alpha(s)}{\nu(s)} \\*
	& \qquad \iN{t}{N}, \iN{s}{d} \\
	& \\
		g(t,s)	& \coloneqq g\left(t, \wt Y_{t-1}^s, \wt Y_{t-2}^s, \wt Y_{t-3}^s, x_{\text{elev},s}, x_{\text{long},s}, x_{\text{lat},s} \sepi \bbeta_\text{ls}\right) \\*
						& \coloneqq \beta_0(s) + \beta_{\sin}(s) \sin\left(\frac{2\pi t}{365.25}\right)
								+ \beta_{\cos}(s) \cos\left(\frac{2\pi t}{365.25}\right)	\\*
						&		+ \gamma_1(s) \wt Y_{t-1}^s + \gamma_2(s) \wt Y_{t-2}^s + \gamma_3(s) \wt Y_{t-3}^s	\\
	& \\
	\beta_{0}(s)	& \coloneqq \beta_{00} + \sum_{j=1}^1{\beta_{01j} x_{\text{elev},s}^j} + \sum_{l=1}^1{\beta_{03l} x_{\text{lat},s}^l}	\\
	\beta_{\sin}(s)	& \coloneqq \beta_{\sin0} + \sum_{j=1}^4{\beta_{\sin1j} x_{\text{elev},s}^j} + \sum_{k=1}^1{\beta_{\sin2k} x_{\text{long},s}^k} + \sum_{l=1}^6{\beta_{\sin3l} x_{\text{lat},s}^l}	\\
	\beta_{\cos}(s)	& \coloneqq \beta_{\cos0} + \sum_{j=1}^6{\beta_{\cos1j} x_{\text{elev},s}^j} + \sum_{k=1}^2{\beta_{\cos2k} x_{\text{long},s}^k} + \sum_{l=1}^1{\beta_{\cos3l} x_{\text{lat},s}^l}	\\
	\gamma_{1}(s)	& \coloneqq \gamma_{10} + \sum_{j=1}^1{\gamma_{11j} x_{\text{elev},s}^j} + \sum_{k=1}^2{\gamma_{12k} x_{\text{long},s}^k} + \sum_{l=1}^6{\gamma_{13l} x_{\text{lat},s}^l}	\\
	\gamma_{2}(s)	& \coloneqq \gamma_{20} + \sum_{j=1}^1{\gamma_{21j} x_{\text{elev},s}^j} + \sum_{k=1}^2{\gamma_{22k} x_{\text{long},s}^k} + \sum_{l=1}^6{\gamma_{23l} x_{\text{lat},s}^l}	\\
	\gamma_{3}(s)	& \coloneqq \gamma_{30} + \sum_{k=1}^4{\gamma_{32k} x_{\text{long},s}^k} + \sum_{l=1}^7{\gamma_{33l} x_{\text{lat},s}^l}	\\	
	\xi(s)	& \coloneqq \xi_{0} + \sum_{j=1}^1{\xi_{1j} x_{\text{elev},s}^j} + \sum_{k=1}^2{\xi_{2k} x_{\text{long},s}^k} + \sum_{l=1}^1{\xi_{3l} x_{\text{lat},s}^l}	\\
	\omega(s)	& \coloneqq \exp\left\{\omega_{0} + \sum_{j=1}^3{\omega_{1j} x_{\text{elev},s}^j} + \sum_{k=1}^1{\omega_{2k} x_{\text{long},s}^k} + \sum_{l=1}^6{\omega_{3l} x_{\text{lat},s}^l}\right\}	\\
	\alpha(s)	& \coloneqq \alpha_{0} + \sum_{j=1}^4{\alpha_{1j} x_{\text{elev},s}^j} + \sum_{k=1}^2{\alpha_{2k} x_{\text{long},s}^k} + \sum_{l=1}^1{\alpha_{3l} x_{\text{lat},s}^l}	\\
	\nu(s)	& \coloneqq \exp\left\{\nu_{0} + \sum_{j=1}^2{\nu_{1j} x_{\text{elev},s}^j} + \sum_{k=1}^2{\nu_{2k} x_{\text{long},s}^k} + \sum_{l=1}^4{\nu_{3l} x_{\text{lat},s}^l}\right\}
\end{align*}
}}

An extensive analysis of the structure of an (truncated\footnote{We considered a truncation after tree ten.}) R-vine copula fitted to the data led to a first new model for spatial dependencies, the spatial R-vine model. The investigation of the relationship between the Kendall's $\tau$ values occurring in the R-vine copula and the distances and elevation differences which can be associated to these Kendall's $\tau$'s proposed different kinds of tree-wise reparametrizations of the first copula parameters. We found that the explanatory power of the elevation differences is comparatively small, whereas the station distances are able to explain the respective correlations to a big extent. This induced the selection of a reparametrization which accounts for all distances between the observation stations which are associated to the respective bivariate copulae of the R-vine copula specification. Moreover a reparametrization of the second copula parameters $\wt\nu_{i(e),j(e)|\calD_e}^l$ depending on the tree number $\iN{l}{10}$ is applied. All in all the selected reparametrizations led to a reduction from $733$ parameters (truncated R-vine copula) to $41$ parameters. They are summarized subsequently.\\

\noindent\fbox{\parbox[l]{0.985\textwidth}{
\noindent\textbf{spatial R-vine model (SV):}\\
\begin{align*}
	\wt\te_{i(e),j(e)|\calD_e}^l	& = g_{l}^{\text{dist}}\left(d_{i(e),j(e)},\ov{d_{i(e),\calD_{e}}},\ov{d_{j(e),\calD_{e}}}|\bbeta_{\text{dist},l},t_{i(e),j(e)|\calD_e}	\right)\\*
						& = \itau\left(\Fzi \left(h_{l}^{\text{dist}}(e|\bbeta_{\text{dist},l})\right);t_{i(e),j(e)|\calD_e}\right), \quad e\in\edge_l, \quad \iN{l}{10} \\
	& \\
	h_{1}^{\text{dist}}\left(e|\bbeta_{\text{dist},1}\right)	&	= \beta_{1,0}^{\text{dist}} + \beta_{1,1}^{\text{dist}}\lnf{d_{i(e),j(e)}}, \quad e\in\edge_1 \\
	h_{l}^{\text{dist}}\left(e|\bbeta_{\text{dist},l}\right)	&	= \beta_{l,0}^{\text{dist}} + \beta_{l,1}^{\text{dist}}\lnf{d_{i(e),j(e)}}	\\*
		& + \beta_{l,2}^{\text{dist}}\lnf{\ov{d_{i(e),\calD_{e}}}}	+ \beta_{l,3}^{\text{dist}}\lnf{\ov{d_{j(e),\calD_{e}}}}, \quad e\in\edge_l, \quad l=2,\ldots,10 \\
	& \\
	\wt\nu_{i(e),j(e)|\calD_e}^l	&	= \exp\left\{(1,l,l^2)\cdot\bbeta_\nu^{\text{SV}}\right\}, \quad e\in\edge_l, \quad \iN{l}{10}
\end{align*}
}}

\clearpage

Our second spatial dependency model is built on the theory of composite likelihood methods. In a first step the model structure, a composition of C-vine copulae, is set up, which results in the definition of a composite vine model. For each variable $u_t^s$ under consideration we determined the three closest\footnote{in terms of station distance} variables denoted as $u^{p_s}_{t}$, $u^{q_s}_{t}$ and $u^{r_s}_{t}$, to set up the four dimensional C-vines composing the model. The resulting components $\calL_s$ of the composite likelihood $\calL_{\text{CVM}}$ and the respective weights $w_s$ are given in the following box.\\

\noindent\fbox{\parbox[l]{0.985\textwidth}{
\noindent\textbf{composite vine model (CVM):}\\
\beqo
	\Lik{\text{CVM}}{\btheta^{\text{CVM}}, \bnu^{\text{CVM}}}{\bu^1,\ldots,\bu^d}	=	\prodsd\prodtN\left[\Lik{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}\right]^{w_s}
\eeqo
with
\begin{align*}
	\Lik{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}	& =	\cop{s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t} \sepi \btheta_s, \bnu_s}	\\*
	& = \cop{sp_s}{u^{s}_{t},u^{p_s}_{t} \sepi \te_{sp_s},\nu_{sp_s}}	\\*
	& \cdot \cop{sq_s}{u^{s}_{t},u^{q_s}_{t} \sepi \te_{sq_s},\nu_{sq_s}}	\\*
	& \cdot	\cop{sr_s}{u^{s}_{t},u^{r_s}_{t} \sepi \te_{sr_s},\nu_{sr_s}}	\\*
	& \cdot	\cop{p_sq_s;s}{\breve{u}^{p_s}_{t},\breve{u}^{q_s}_{t} \sepi \te_{p_sq_s|s},\nu_{p_sq_s|s}}	\\*
	& \cdot \cop{p_sr_s;s}{\breve{u}^{p_s}_{t},\breve{u}^{r_s}_{t} \sepi \te_{p_sr_s|s},\nu_{p_sr_s|s}}	\\*
	& \cdot	\cop{q_sr_s;sp_s}{\check{u}^{q_s}_{t},\check{u}^{r_s}_{t} \sepi \te_{q_sr_s|sp_s},\nu_{q_sr_s|sp_s}}, \quad\iN{t}{N} \\
	& \\
	\breve{u}^{o}_{t} =	F(u^{o}_{t} \sep u^{s}_{t})	& =	\partialderiv{u^{s}_{t}} \Cop{os}{u^{o}_{t},u^{s}_{t} \sepi \te_{so},\nu_{so}}, \quad o=p_s,q_s,r_s	\\
	\check{u}^{o}_{t} =	F(u^{o}_{t} \sep u^{s}_{t},u^{p_s}_{t})	& = \partialderiv{\breve{u}^{p_s}_{t}} \Cop{op_s;s}{\breve{u}^{o}_{t},\breve{u}^{p_s}_{t} \sepi \te_{p_so|s},\nu_{p_so|s}}, \quad o=q_s,r_s	\\
	& \\
	d	& =	\# \mbox{ of components}	\\
	N	& =	\# \mbox{ of observations}	\\
\end{align*}
and weights
\beqo
	w_s \coloneqq \frac{1}{n_s}, \quad\text{with}\quad n_s \coloneqq \#\left\{k: s \mbox{ is included in C-vine }k\right\},\ \iN{s}{d}
\eeqo
}}

\clearpage

We subsequently investigated a fit of the resulting composite vine model to the data in a similar way as for the spatial R-vine model. Again different reparametrizations were compared. This time we decided to account additionally to the distances for the elevation differences in the joint reparametrization of the first copula parameters of the first C-vine trees. The second and third tree copula reparametrizations account furthermore only for the occurring distances as predictors. The reparametrization of the second copula parameters depends on the tree number $\iN{l}{10}$ and the distances indicated by the respective conditioned sets. Whereas the composite vine model is based on $495$ parameters, this number could be reduced to $16$ for the reparametrized composite vine model, the spatial composite vine model. It is summarized in the following box.\\

\noindent\fbox{\parbox[l]{0.985\textwidth}{
\noindent\textbf{spatial composite vine model (SCVM):}\\
\begin{align*}
	\wt\te_{so_1}	&	= \itau\left(\Fzi \left(h_{1}^{\text{select}}(s,o_1|\bbeta_{\text{select},1})\right);t_{so_1}\right) \\*
	\wt\te_{p_so_2|s}	&	= \itau\left(\Fzi \left(h_{2}^{\text{select}}(s,p_s,o_2|\bbeta_{\text{select},2})\right);t_{p_so_2|s}\right)	\\*
	\wt\te_{q_sr_s|sp_s}	&	= \itau\left(\Fzi \left(h_{3}^{\text{select}}(s,p_s,q_s,r_s|\bbeta_{\text{select},3})\right);t_{q_sr_s|sp_s}\right),	\qquad \iN{s}{d}	
\end{align*}
\begin{align*}
	h_{1}^{\text{select}}\left(s,o_1|\bbeta_{\text{select},1}\right) = \beta_{1,0}^{\text{select}}	&	+ \beta_{1,1}^{\text{select}}\lnf{d_{s,o_1}} + \beta_{1,2}^{\text{select}}\lnf{e_{s,o_1}}	\\
	h_{2}^{\text{select}}\left(s,p_s,o_2|\bbeta_{\text{select},2}\right) = \beta_{2,0}^{\text{select}}	&	+ \beta_{2,1}^{\text{select}}\lnf{d_{p_s,o_2}}	+ \beta_{2,2}^{\text{select}}\lnf{d_{p_s,s}}	+ \beta_{2,3}^{\text{select}}\lnf{d_{o_2,s}}	\\
	h_{3}^{\text{select}}\left(s,p_s,q_s,r_s|\bbeta_{\text{select},3}\right) = \beta_{3,0}^{\text{select}}	&	+ \beta_{3,1}^{\text{select}}\lnf{d_{q_s,r_s}}	+ \beta_{3,2}^{\text{select}}\lnf{d_{q_s,s}}	+ \beta_{3,3}^{\text{select}}\lnf{d_{q_s,p_s}}	\\*
				&	+ \beta_{3,4}^{\text{select}}\lnf{d_{r_s,s}}	+ \beta_{3,5}^{\text{select}}\lnf{d_{r_s,p_s}}
\end{align*}
\begin{align*}
	\wt\nu_{so_1}	&	= \exp\left(\beta_{0}^{\nu} + \beta_{1}^{\nu}\cdot1 + \beta_{2}^{\nu}d_{s,o_1}\right)	\\*
	\wt\nu_{p_so_2|s}	&	= \exp\left(\beta_{0}^{\nu} + \beta_{1}^{\nu}\cdot2 + \beta_{2}^{\nu}d_{p_s,o_2}\right)	\\*
	\wt\nu_{q_sr_s|sp_s}	&	= \exp\left(\beta_{0}^{\nu} + \beta_{1}^{\nu}\cdot3 + \beta_{2}^{\nu}d_{q_s,r_s}\right)	
\end{align*}
\begin{align*}
	o_1	&	= p_s,q_s,r_s\\*
	o_2	&	= q_s,r_s
\end{align*}
}}

\clearpage

For the purpose of model evaluation and comparison a third spatial model was introduced, the spatial Gaussian model, which models the spatial dependencies based on a Gaussian variogram model and assumes a multivariate Gaussian distribution of the mean temperatures.\\

\noindent\fbox{\parbox[l]{0.985\textwidth}{
\textbf{spatial Gaussian model (SG):}\\
\beqo
	\wt \bY_t = \bmu_t + \bveps_t, \quad \bveps_t\simiid\mvN{d}{\bnull}{\Sigma(\btheta^{\text{SG}})}, \quad \iN{t}{N}
\eeqo
\begin{align*}
		\mu_t^s	&	\coloneqq g(t,s) = g\left(t, \wt Y_{t-1}^s, \wt Y_{t-2}^s, \wt Y_{t-3}^s, x_{\text{elev},s}, x_{\text{long},s}, x_{\text{lat},s} \sepi \bbeta_\text{ls}\right) \\*
						& \coloneqq \beta_0(s) + \beta_{\sin}(s) \sin\left(\frac{2\pi t}{365.25}\right)
								+ \beta_{\cos}(s) \cos\left(\frac{2\pi t}{365.25}\right)	\\*
						&		+ \gamma_1(s) \wt Y_{t-1}^s + \gamma_2(s) \wt Y_{t-2}^s + \gamma_3(s) \wt Y_{t-3}^s	\qquad \mbox{(compare marginal model)}	\\
	& \\
	\gamma(h \sepi \eta, \varsigma, \rho)	& \coloneqq \varsigma\left(1-\exp\left(-\frac{h^2}{\rho^2}\right)\right) + \eta{\mathds 1}_{(0,\infty)}(h)	\qquad \mbox{(Gaussian variogram model)}	\\
	& \\
	\Sigma_{i,j}(\btheta^{\text{SG}})	& \coloneqq \sigma^2 - \gamma(d_{i,j} \sepi \eta, \varsigma, \rho)	\\
	& \\
\wh\bveps_t	& \coloneqq \wt\by_t-\wh\bmu_t(\wh\bbeta_\text{ls})
\end{align*}
}}\\

An overview and comparison of all dependency models under consideration is given by Tables \ref{tab:mov1}-\ref{tab:mov3}. Amongst others, the likelihood-functions corresponding to the models summarized above are given.\footnote{$\wt{u}^{i(e)}_t = F_{i(e)|\calD_e}(u^{i(e)}_t\sep\bu^{\calD_e}_t), ~\wt{u}^{j(e)}_t = F_{j(e)|\calD_e}(u^{j(e)}_t\sep\bu^{\calD_e}_t), ~\bu^{\calD_e}_t \coloneqq \left\{u_t^s: s\in\calD_e\right\}$}$^,$\footnote{Reparametrized parameters are indicated by a tilde.}


%\noindent\fbox{\parbox[l]{0.985\textwidth}{
%\noindent\textbf{full R-vine model (RV):}\\
%\begin{align*}
	%\Lik{\text{RV}}{\btheta^{\text{RV}}, \bnu^{\text{RV}}}{\bu^1,\ldots,\bu^d}	&	= \prod_{t=1}^N\prod_{l=1}^{d-1}\prod_{e\in\edge_l} \cop{i(e),j(e);\calD_e}{\wt{u}^{i(e)}_t ,\wt{u}^{j(e)}_t\sepi\te_{i(e),j(e)|\calD_e},\nu_{i(e),j(e)|\calD_e},t_{i(e),j(e)|\calD_e}}, \\
	%\wt{u}^{i(e)}_t	&	= F_{i(e)|\calD_e}(u^{i(e)}_t\sep\bu^{\calD_e}_t),	\\
	%\wt{u}^{j(e)}_t	&	= F_{j(e)|\calD_e}(u^{j(e)}_t\sep\bu^{\calD_e}_t),	\\
	%\bu^{\calD_e}_t	&	\coloneqq \left\{u_t^s: s\in\calD_e\right\}.
%\end{align*}
%}}
%
%\noindent\fbox{\parbox[l]{0.985\textwidth}{
%\noindent\textbf{truncated R-vine model (TRV):}\\
%\begin{align*}
	%\Lik{\text{TRV}}{\btheta^{\text{TRV}}, \bnu^{\text{TRV}}}{\bu^1,\ldots,\bu^d}	&	= \prod_{t=1}^N\prod_{l=1}^{10}\prod_{e\in\edge_l} \cop{i(e),j(e);\calD_e}{\wt{u}^{i(e)}_t ,\wt{u}^{j(e)}_t\sepi\te_{i(e),j(e)|\calD_e},\nu_{i(e),j(e)|\calD_e},t_{i(e),j(e)|\calD_e}}, \\
	%\wt{u}^{i(e)}_t	&	= F_{i(e)|\calD_e}(u^{i(e)}_t\sep\bu^{\calD_e}_t),	\\
	%\wt{u}^{j(e)}_t	&	= F_{j(e)|\calD_e}(u^{j(e)}_t\sep\bu^{\calD_e}_t),	\\
	%\bu^{\calD_e}_t	&	\coloneqq \left\{u_t^s: s\in\calD_e\right\}.
%\end{align*}
%}}



\begin{landscape}
\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{p{1.2cm}|p{2cm}p{3cm}p{1.2cm}p{2.1cm}p{1.6cm}p{2.5cm}}
%			&		&		&		&	model is based	&		&		&		&	maximum	&		&		&		&		\\
%		short	&	full	&	model	&	trunc.	&	on spatial	&	data	&	parameters	&	$\#$par	&	(composite)			&	AIC	&	BIC	&	computation	&	likelihood-	\\
		short name	&	full name	&	model type	&	trunc. level	&	model is \newline based on \newline spatial \newline information	&	data level	&	parameters	\\
		\hline
		\hline
		RV	&	full R-vine	&	vine copula	&	$-$	&	no	&	copula data	&	$\btheta^{\text{RV}}, \bnu^{\text{RV}}$	\\
		TRV	&	truncated \newline R-vine	&	truncated \newline vine copula	&	10	&	no	&	copula data	&	$\btheta^{\text{TRV}}, \bnu^{\text{TRV}}$	\\
		SV	&	spatial \newline R-vine	&	reparametrized \newline truncated \newline vine copula	&	10	&	yes	&	copula data	&	$\bbeta_{\text{dist}}^{\text{SV}}, \bbeta_\nu^{\text{SV}}$	\\
		\hline
		\hline
		CVM	&	composite \newline vine model	&	composite \newline likelihood \newline model	&	$-$	&	(for model \newline structure)	&	copula data	&	$\btheta^{\text{CVM}}, \bnu^{\text{CVM}}$	\\
		SCVM	&	spatial \newline composite \newline vine model	&	reparametrized \newline composite \newline likelihood \newline model	&	$-$	&	yes	&	copula data	&	$\bbeta_{\text{select}}^{\text{SCVM}}, \bbeta_\nu^{\text{SCVM}}$	\\
		\hline
		\hline
		SG	&	spatial \newline Gaussian \newline model	&	semivariogram \newline based	&	$-$ & yes	&	residuals	&	$\btheta^{\text{SG}}$	
		\end{tabular}
	\end{center}
	\caption{Model overview: model type, used truncation level, usage of spatial information, data level on which the models are fitted and the model parameters.}
	\label{tab:mov1}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{p{1.2cm}|p{2cm}p{18cm}}
		short name	&	full name	&	likelihood-function	\\
		\hline
		\hline
		RV	&	full R-vine	&	\parbox[l]{18cm}{\beqo\Lik{\text{RV}}{\btheta^{\text{RV}}, \bnu^{\text{RV}}}{\bu^1,\ldots,\bu^d} = \prod_{t=1}^N\prod_{l=1}^{d-1}\prod_{e\in\edge_l} \cop{i(e),j(e);\calD_e}{\wt{u}^{i(e)}_t ,\wt{u}^{j(e)}_t\sepi\te_{i(e),j(e)|\calD_e},\nu_{i(e),j(e)|\calD_e},t_{i(e),j(e)|\calD_e}}\eeqo}	\\
		TRV	&	truncated \newline R-vine	&	\parbox[l]{18cm}{\beqo\Lik{\text{TRV}}{\btheta^{\text{TRV}}, \bnu^{\text{TRV}}}{\bu^1,\ldots,\bu^d} = \prod_{t=1}^N\prod_{l=1}^{10}\prod_{e\in\edge_l} \cop{i(e),j(e);\calD_e}{\wt{u}^{i(e)}_t ,\wt{u}^{j(e)}_t\sepi\te_{i(e),j(e)|\calD_e},\nu_{i(e),j(e)|\calD_e},t_{i(e),j(e)|\calD_e}}\eeqo}	\\
		SV	&	spatial \newline R-vine	&	\parbox[l]{18cm}{\beqo\Lik{\text{SV}}{\bbeta_{\text{dist}}^{\text{SV}}, \bbeta_\nu^{\text{SV}}}{\bu^1,\ldots,\bu^d} 	= \prod_{t=1}^N\prod_{l=1}^{10}\prod_{e\in\edge_l} \cop{i(e),j(e);\calD_e}{\wt{u}^{i(e)}_t ,\wt{u}^{j(e)}_t\sepi\wt\te_{i(e),j(e)|\calD_e}^l,\wt\nu_{i(e),j(e)|\calD_e}^l,t_{i(e),j(e)|\calD_e}}\eeqo}	\\
		\hline
		\hline
		CVM	&	composite \newline vine model	&	\parbox[l]{18cm}{\beqo\Lik{\text{CVM}}{\btheta^{\text{CVM}}, \bnu^{\text{CVM}}}{\bu^1,\ldots,\bu^d}	=	\prodsd\prodtN\left[\Lik{s}{\btheta_s, \bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}\right]^{w_s}\eeqo}	\\
		SCVM	&	spatial \newline composite \newline vine model	&	\parbox[l]{18cm}{\beqo\Lik{\text{SCVM}}{\bbeta_{\text{select}}^{\text{SCVM}}, \bbeta_\nu^{\text{SCVM}}}{\bu^1,\ldots,\bu^d}	=	\prodsd\prodtN\left[\Lik{s}{\wt\btheta_s, \wt\bnu_s}{u^{s}_{t},u^{p_s}_{t},u^{q_s}_{t},u^{r_s}_{t}}\right]^{w_s}\eeqo}	\\
		\hline
		\hline
		SG	&	spatial \newline Gaussian \newline model	&	\parbox[l]{18cm}{\beqo\Lik{\text{SG}}{\btheta^{\text{SG}}}{\xn{\wh\bveps}{N}} = \prodtN\frac{1}{\sqrt{(2\pi)^{d}\left|\Sigma(\btheta^{\text{SG}})\right|}}\exp\left\{-\half\wh\bveps_t\T\left[\Sigma(\btheta^{\text{SG}})\right]^{-1}\wh\bveps_t\right\}\eeqo}
		\end{tabular}
	\end{center}
	\caption{Model overview: likelihood-functions corresponding to the models summarized above.}
	\label{tab:mov2}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{p{1.2cm}|p{2cm}p{2.3cm}p{2cm}p{2cm}p{1cm}p{2.5cm}}
		short name	&	full name	&	maximum \newline (composite) \newline log-likelihood	&	AIC	&	BIC	&	$\#$par	&	computation time	\\
		\hline
		\hline
		RV	&	full R-vine	&	62714.19	&	-121856.4	&	-112932.3	&	1786	&	$\sim$ 54 days	\\
		TRV	&	truncated \newline R-vine	&	58366.70	&	-115267.4	&	-111604.8	&	733	&	$\sim$ 3.7 days	\\
		SV	&	spatial \newline R-vine	&	54650.11	&	-109218.2	&	-109013.4	&	41	&	$\sim$ 18 h	\\
		\hline
		\hline
		CVM	&	composite \newline vine model	&	42106.41	&	-83222.8	&	-80749.5	&	495	&	$\sim$ 6.1 days	\\
		SCVM	&	spatial \newline composite \newline vine model	&	40938.80	&	-81845.6	&	-81765.7	&	16	&	$\sim$ 1.6 h	\\
		\hline
		\hline
		SG	&	spatial \newline Gaussian \newline model	&	-50007.76	&	100023.5	&	100043.5	&	4	&	$\sim$ 5.3 min
		\end{tabular}
	\end{center}
	\caption{Model overview: maximum (composite) log-likelihood, AIC, BIC, number of parameters needed, elapsed computation time.}
	\label{tab:mov3}
\end{table}
\end{landscape}

The prediction results from all three models were quite similar and reasonable, as long as the location from which we aimed to predict lay within the range of the training data. In order to rank the different model predictions, we calculated and compared continuous ranked probability scores and interval scores. In terms of both scores we observed an outperformance of our two vine copula based spatial dependency models over the spatial Gaussian model. Direct comparison of the spatial R-vine model and the spatial composite vine model yielded an outperformance of the spatial R-vine model with regard to the continuous ranked probability scores and an outperformance of the spatial composite vine model with respect to the interval scores.

Whereas the prediction from our spatial R-vine model uses the information of all $54$ observation stations of the training data set, the spatial composite vine model based predictions are only conditioned on the observations of three neighboring stations. These differences in the model structure naturally have an effect with regard to computation time. Therefore, further investigations of the performance of spatial composite vine models which consider different numbers of neighboring stations are of big interest. Moreover an application of our modeling approaches to other types of data sets is desirable, which implicitly requires the development of new marginal models. Especially an investigation of data sets where asymmetries of bivariate dependencies are observed should stand in the focus of further work on this topic.

\cleardoublepage

